Privately Publishable Per-instance Privacy

We consider how to privately share the personalized privacy losses incurred by objective perturbation, using per-instance differential privacy (pDP). Standard differential privacy (DP) gives us a worst-case bound that might be orders of magnitude larger than the privacy loss to a particular individual relative to a fixed dataset. The pDP framework provides a more fine-grained analysis of the privacy guarantee to a target individual, but the per-instance privacy loss itself might be a function of sensitive data. In this paper, we analyze the per-instance privacy loss of releasing a private empirical risk minimizer learned via objective perturbation, and propose a group of methods to privately and accurately publish the pDP losses at little to no additional privacy cost.

==> Privately Publishable Per-instance Privacy/abstract.tex <==
% !TEX root = ../main.tex

    \begin{abstract}
We consider how to privately share the personalized privacy losses incurred by objective perturbation, using per-instance differential privacy (pDP). Standard differential privacy (DP) gives us a worst-case bound that might be orders of magnitude larger than the privacy loss to a particular individual relative to a fixed dataset. The pDP framework provides a more fine-grained analysis of the privacy guarantee to a target individual, but the per-instance privacy loss itself might be a function of sensitive data. In this paper, we analyze the per-instance privacy loss of releasing a private empirical risk minimizer learned via objective perturbation, and propose a group of methods to privately and accurately publish the pDP losses at little to no additional privacy cost.    \end{abstract}


==> Privately Publishable Per-instance Privacy/sections/conclusion.tex <==
% !TEX root = ../main.tex

We precisely calculate the privacy loss that an individual $z$ suffers \emph{after} the objective perturbation algorithm is run on a specific dataset. The \emph{ex-post} pDP loss function in DP-ERM can be accurately released to all individuals with little or
no additional privacy cost. In particular, we present a \emph{data-independent} bound which empirically provides a reasonably accurate estimate of the \emph{ex-post} pDP loss while requiring no further privatization step. Reserving some of the privacy budget allows us to alternatively release a tighter \emph{data-dependent} bound.

An important next step is to extend the per-instance DP analysis to the setting of constrained optimization. There are many promising future directions including using publishable pDP losses for designing more data-adaptive DP algorithms.
%In this work we show how to privately and accurately release the personalized privacy losses incurred by the objective perturbation mechanism. Our theoretical and experimental results demonstrate that our methods provide strong, adaptive privacy guarantees applicable to a wide range of learning problems, and that we can release privatized pDP losses which are good approximations of the true pDP losses.

%Objective perturbation is merely one among many potential applications of pDP made practical. The pDP framework can easily accommodate a wide variety of privacy needs and learning algorithms. We’ve shown already that it can adapt to the dataset, to individuals both in and out of the dataset, and to the realization of the private output of the mechanism. As future work, the pDP framework could even adapt to a particular set of colluding adversaries. Other future directions include extending the framework to handle constrained optimization and using the pDP analysis for designing new data-adaptive DP algorithms.


% Our framework applies to a wide range of learning problems, but our pDP analysis limits us to unconstrained optimization. In future work we will explore how to extend our approach to optimization over any convex domain.


==> Privately Publishable Per-instance Privacy/sections/experiments.tex <==
% !TEX root = ../main.tex

Here we evaluate our methods to release the pDP losses using logistic regression as a case study. In Section ~\ref{reg_utility}, we demonstrate that the stronger regularization required by Algorithm ~\ref{alg:privacy_report} does not affect the utility of the model. In Section ~\ref{dep_indep_compare} we show that by carefully allocating the privacy budget of the data-dependent release, we can achieve a more accurate estimate of the \emph{ex-post} pDP losses of Algorithm ~\ref{alg:Alg1} compared to the data-independent release, with reasonable overhead (same overall DP budget and only a slight uptick in the overall pDP losses).

Experiments with linear regression, with additional datasets and with alternative privacy budget allocation schemes are included in the supplementary materials.
%\textbf{Experimental Setup}\: 
%Throughout, we set $\delta = 10^{-6}$ (failure probability of Algorithm ~\ref{alg:Alg1}, i.e. objective perturbation) and $\rho = 10^{-6}$ (failure probability of Algorithm \ref{alg:privacy_report} that releases a private upper bound on the pDP loss). Our choice of $\sigma$ depends on $\epsilon_1$ and follows the requirements for objective perturbation stated in Theorem \ref{thm:alg1} to achieve DP.  Unless otherwise specified, we set $\lambda$ as described in Algorithm \ref{alg:privacy_report}. We don't use any additional regularization, i.e. $r(\theta) = 0$. The noise parameters $\sigma_2, \sigma_3$ are each calibrated according to the analytic Gaussian mechanism of \citep{balle2018improving}, with an equal privacy budget allotted to each private release. In other words, Algorithm \ref{alg:Alg1} which releases $\hat{\theta}^P$ has a budget of $\epsilon_1$; Algorithm \ref{alg:privacy_report} which releases $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$ has a budget of $2\epsilon_1$; and therefore the combined privacy budget of objective perturbation and releasing the associated pDP losses is equal to $3 \epsilon_1$.

%\textbf{Datasets}
% Section ~\ref{reg_utility} In Section ~\ref{dep_indep_compare}, we evaluate our methods on the credit card default dataset \citep{yeh2009comparisons} from the UCI Machine Learning Repository.
%kidney, synthetic, credit, liver, wine
%For experiments related to linear regression, we use the wine quality dataset \citep{Dua:2019} from the UCI Machine Learning Repository. We also evaluate our methods on synthetic data generated by sampling $x_i, \theta \sim \mathcal{N}(0, I_d)$ and normalizing each $x_i \in X$ so that $||x_i||_2 = 1$. The unperturbed response variable $Y \in \mathbb{R}^n$ is then determined as $Y = X \theta$ and rescaled so that each $y_i \in [0, 1]$.
%We use three UCI datasets to test our methods on logistic regression: the credit card default dataset \citep{yeh2009comparisons}, the chronic kidney disease dataset and the liver disorders dataset \citep{Dua:2019}. In addition, we generate synthetic data by sampling  $x_i, \theta \sim \mathcal{N}(0, I_d)$ and determining each $y_i$ as
%\centerline{
% $$y_i = \begin{cases} 
%         1 & \text{ if } \texttt{sigmoid}(x_i^T\theta) > 0.5, \\ 
%         0 & \text{ otherwise.} \end{cases}$$
%         %}
\subsection{Stronger regularization does not worsen model utility}
\label{reg_utility}

In this experiment we use a synthetic dataset generated by sampling $x_i, \theta \sim \mathcal{N}(0, I_d)$ and normalizing each $x_i \in X$ so that $||x_i||_2 = 1$. Then we rescale $Y = X \theta$ to ensure $y_i \in [0, 1]$ for each $y_i \in Y$. \newline\newline
% logistic regression
% explain lambda_inflate
% star denotes the actual inflation value (how many times larger \lambda_{adapt} is than \lambda_{obj})
\begin{minipage}{.4\textwidth}
Algorithm ~\ref{alg:privacy_report} requires a larger $\lambda$ than suggested by Theorem $\ref{thm:alg1}$ in order to achieve a uniform multiplicative approximation of $\mu(\cdot)$.  
We investigate the effect of stronger regularization on the utility of a private logistic regression model applied to a synthetic dataset ($n = 1000, d = 50$), for several settings of $\epsilon_1$. Since each value of $\epsilon_1$ demands a different minimum value of $\lambda$ in order to achieve $(\epsilon_1, \delta)$-differential privacy, we compare via "$\lambda$-inflation": a measure of how many times larger we set $\lambda$ than its minimum value required to achieve the worst-case DP bound of objective perturbation.
\end{minipage}
\hspace{.2cm}\begin{minipage}{.6\textwidth}
\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/lambda_utility.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Utility of Obj-Pert with larger $\lambda$.}
  \label{fig:lambda_utility}
\end{figure}
\end{minipage}

  E.g., for logistic regression the objective perturbation mechanism requires $\lambda \geq \frac{1}{2\epsilon}$, and so in Figure ~\ref{fig:lambda_utility} a $\lambda$-inflation value of 10 means that we set $\lambda = \frac{5}{\epsilon}$. For each $\lambda$-inflate value $c$ , we run Algorithm \ref{alg:Alg1} with $\lambda = c \lambda_{\texttt{Obj-Pert}}$.  In particular, the star symbol marks the level of $\lambda$-inflation enforced by Algorithm ~\ref{alg:privacy_report}. The experimental results summarized in Figure ~\ref{fig:lambda_utility} show that the performance of the private logistic regression model (as measured by the 0-1 loss) remains roughly constant across varying scales of $\lambda$.


\subsection{Comparison of data-independent and data-dependent bounds}
\label{dep_indep_compare}

The following experiments feature the credit card default dataset ($n = 30000, d = 21$) \citep{yeh2009comparisons} from the UCI Machine Learning Repository. We privately train a binary classifier to predict whether or not a credit card client $z$ defaults on her payment (Algorithm \ref{alg:Alg1}), and calculate the true pDP loss $\epsilon_1(\cdot)$ as well as the data-independent and -dependent estimates $\overline{\epsilon_1^P}(\cdot)$ for each $z$ in the training set (Algorithm \ref{alg:privacy_report}).



% Sections ~\ref{total_privacy_same} and ~\ref{equal_allocation} differ only in the allocation of the privacy budget. 
%Throughout, we set $\delta = 10^{-6}$ (failure probability of Algorithm ~\ref{alg:Alg1}, i.e. objective perturbation) and $\rho = 10^{-6}$ (failure probability of Algorithm \ref{alg:privacy_report} that releases a private upper bound on the pDP loss). Our choice of $\sigma$ depends on $\epsilon_1$ and follows the requirements for objective perturbation stated in Theorem \ref{thm:alg1} to achieve DP.  Unless otherwise specified, we set $\lambda$ as described in Algorithm \ref{alg:privacy_report}. We don't use any additional regularization, i.e. $r(\theta) = 0$. The noise parameters $\sigma_2, \sigma_3$ are each calibrated according to the analytic Gaussian mechanism of \citep{balle2018improving}, with an equal privacy budget allotted to each private release. In other words, Algorithm \ref{alg:Alg1} which releases $\hat{\theta}^P$ has a budget of $\epsilon_1$; Algorithm \ref{alg:privacy_report} which releases $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$ has a budget of $2\epsilon_1$; and therefore the combined privacy budget of objective perturbation and releasing the associated pDP losses is equal to $3 \epsilon_1$.
The failure probabilities for both Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report} are set as $\delta = \rho = 10^{-6}$. Our choices of $\sigma$ and $\lambda$ depend on $\epsilon_1$ and follows the requirements stated in Theorem \ref{thm:alg1} to achieve DP. We don't use any additional regularization, i.e. $r(\theta) = 0$. For the data-dependent release, the noise parameters $\sigma_2, \sigma_3$ are each calibrated according to the analytic Gaussian mechanism of \citep{balle2018improving}.

Using $\epsilon = 1$ as a DP budget, we investigate how to allocate the privacy budget among the components of the data-dependent release ($\epsilon = \epsilon_1 + \epsilon_2 + \epsilon_3$) to achieve a favorable comparison with the data-independent release which requires no additional privacy cost ($\epsilon = \epsilon_1$). The configuration described in Figure ~\ref{fig:ep1_aligned}, which skews the data-dependent privacy budget toward more accurately releasing $\overline{\epsilon_1^P}(\cdot)$, was empirically chosen as an example where the sum $\overline{\epsilon_1^P}(\cdot) + \epsilon_2(\cdot) + \epsilon_3(\cdot)$ of privately released pDP losses of the data-dependent approach  are comparable to the privately released $\emph{ex-post}$ pDP loss $\overline{\epsilon_1^P}(\cdot)$ of the data-independent approach. Note that $\epsilon_2(\cdot)$ and $\epsilon_3(\cdot)$ aren't $\emph{ex-post}$ in the traditional sense; however, we feel comfortable summing $\overline{\epsilon_1^P}(\cdot) + \epsilon_2(\cdot) + \epsilon_3(\cdot)$ since all three terms are a function of $\hat{\theta}^P$ and individual $z$'s data. Note also that since the total budget $\epsilon$ is the same for both the data-independent and -dependent releases, $\epsilon_1$ differs between them. Therefore Figure ~\ref{fig:comp_ratio} compares the accuracy of both approaches using the ratio between $\overline{\epsilon_1^P}(\cdot)$ and $\epsilon_1(\cdot)$ rather than their raw values.
% \subsubsection{Equal allocation}
% \label{equal_allocation}



\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/align_combined.pdf}
\subfloat[Distribution of privately released \emph{ex-post} pDP losses. \label{fig:ep1_align_raw}]{\hspace{.39\linewidth}}\hspace{1.5cm}
\subfloat[ Distribution of ratios between the privately released \emph{ex-post} pDP losses $\overline{\epsilon_1^P}(\cdot)$ and their true values $\epsilon_1(\cdot)$. \label{fig:comp_ratio}]{\hspace{.35\linewidth}}
  \caption{True and privately released pDP losses when the total privacy budget is $\epsilon = 1$. For the data-independent release we use the entire privacy budget on releasing $\hat{\theta}^P$ ($\epsilon_1 = 1$). For the data-dependent release we reserve some of the privacy budget for releasing $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$ ($\epsilon_1 = 0.2, \epsilon_2 = 0.7, \epsilon_3 = 0.1$).}
  \label{fig:ep1_aligned}
\end{figure}

When including the additional privacy budget incurred by the data-dependent approach, the data-dependent approach loses its competitive edge over the data-independent approach. Note that setting $\epsilon_2 = \epsilon_3 = 0$ would reduce the data-dependent approach to the data-independent one. The real advantage of the data-dependent approach can be best seen by allotting only a small portion of the overall privacy budget to Algorithm ~\ref{alg:Alg1}; then we can release $\hat{\theta}^P$ and $\overline{\epsilon_1^P}(\cdot)$ with reasonable overhead while achieving tighter and more accurate upper bounds for $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$. By suffering a small additional \emph{ex-post} pDP loss (Figure ~\ref{fig:ep1_align_raw}), we can release the \emph{ex-post} pDP losses of Algorithm ~\ref{alg:Alg1} much more accurately (Figure ~\ref{fig:comp_ratio}). The downside to this is that reducing $\epsilon_1$ reduces the accuracy of the output $\hat{\theta}^P$. Deciding how to allocate the privacy budget between $\epsilon_1, \epsilon_2$ and $\epsilon_3$ thus requires weighing the importance of an accurate $\hat{\theta}^P$ against the importance of an accurate $\overline{\epsilon_1^P}(\cdot)$.

% \subsubsection{Total privacy budget is the same}
% \label{total_privacy_same}
% We align the total DP budget $\epsilon_1 + \epsilon_2 + \epsilon_3$ to compare the data-independent and data-dependent bounds, with  $\epsilon_1^{\texttt{DEP}} = 1$ and $\epsilon_1^{\texttt{INDEP}} = 0.2, \epsilon_2^{\texttt{INDEP}} = 0.4, \epsilon_3^{\texttt{INDEP}} = 0.4$. Privacy parameters $\sigma, \lambda, \sigma_2, \sigma_3$ are chosen as described in the experimental setup in the main paper. When including the additional privacy budget incurred by the data-dependent approach, the data-dependent approach loses its competitive edge over the data-independent approach. Note that setting $\epsilon_1^{\texttt{DEP}} = 1, \epsilon_2^{\texttt{DEP}} = 0$ and $\epsilon_3^{\texttt{INDEP}} = 0$ would reduce the data-dependent approach to the data-independent one. The real advantage of the data-dependent approach can be best seen by allotting only a small portion of the overall privacy budget to Algorithm ~\ref{alg:Alg1}; then we can release $\hat{\theta}^P$ with only a small pDP loss while achieving tighter and more accurate upper bounds for $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$. By suffering a small additional pDP loss (Figure ~\ref{fig:data_indep_dep_align}), we can release the pDP losses of Algorithm ~\ref{alg:Alg1} much more accurately (Figure ~\ref{fig:ep1_ratio_align}).
% \label{compare_dep_indep}
% \begin{figure}[H]
%   \centering
% \includegraphics[width=\textwidth]{experiments/align_combined.pdf}
% \subfloat[\label{fig:data_indep_dep_align} Total privacy loss.]{\hspace{.56\linewidth}}
% \subfloat[\label{fig:ep1_ratio_align} Competitive ratio.]{\hspace{.5\linewidth}}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Comparison of data-independent and -dependent upper bounds}
%   \label{fig:ep1_compare}
% \end{figure}


% Algorithm ~\ref{alg:privacy_report} presents two approaches to releasing a private upper bound of $\epsilon_1(\cdot)$, the pDP loss of releasing $\hat{\theta}^P$ from Algorithm ~\ref{alg:Alg1}. The data-independent approach bounds the pDP loss using only individual $z$'s own data as well as publicly-known parameters of the algorithm ($\rho, \sigma, \lambda$). The data-dependent approach privatizes the quantities $\mu(\cdot)$ and $g(\cdot) := \nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)$ that depend on the entire dataset. While the data-dependent approach can more accurately release $\overline{\epsilon_1^P}(\cdot)$, it suffers an additional privacy loss which could negate the savings of a more accurate bound on the pDP loss of Algorithm ~\ref{alg:Alg1}. It is therefore of interest to us to investigate the trade-offs of both approaches.

% First, we run both the data-independent and -dependent variations of Algorithm ~\ref{alg:Alg1} with privacy parameters set to achieve $\epsilon_1 = \epsilon_2 = \epsilon_3 = 1$, as described in the experimental setup. Figure ~\ref{fig:ep1_compare} compares the distributions of the true pDP loss $\epsilon_1(\cdot)$ and its privately released upper bound $\overline{\epsilon_1^P}(\cdot)$ using both the data-independent and -dependent approaches. We see that for the same privacy budget $\epsilon_1 = 1$ allotted to Algorithm ~\ref{alg:Alg1} (indicated by the red line), the data-dependent upper bound is significantly tighter than the data-independent upper bound. However, Figure ~\ref{fig:ep1_compare} doesn't take into account the additional privacy loss incurred by using the data-dependent version of Algorithm ~\ref{alg:privacy_report}.

% \begin{figure}[H]
%   \centering
% \includegraphics[width=\textwidth]{experiments/ep1_datasets.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Comparison of pDP losses and data-independent and -dependent upper bounds}
%   \label{fig:ep1_compare}
% \end{figure}

% Figure ~\ref{fig:ep1_ep23_compare} includes the additional per-instance privacy loss of Algorithm ~\ref{alg:privacy_report} (for the data-independent version, we simply have $\epsilon_2(\cdot) = \epsilon_3(\cdot) = 0$). When considering the combined pDP loss of running Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report}, the data-independent bound is tighter. However, it is perhaps unfair of us to compose the \emph{ex-post} pDP loss of Algorithm ~\ref{alg:Alg1} with the \emph{ex-ante} pDP loss of Algorithm ~\ref{alg:privacy_report}, particularly given that the the \emph{ex-ante} pDP loss of Algorithm ~\ref{alg:privacy_report} has a necessary dependence on the order of $\sqrt{2\log(1/\delta)}$. In the appendix, we explore how to allocate the privacy budget between Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report} in order to achieve a more favorable trade-off between the data-independent and data-dependent approaches.

% Based on our theory and experiments, our recommendation is to use data-independent bounds if $\lambda$ is large (the second or the third term dominates $\epsilon_1(\cdot)$). 
% The data-dependent bound (and the adaptive algorithm presented in the appendix) may be preferred if $\lambda$ is small and the $-\log(1-\mu(\cdot))$ term dominates  the $\epsilon_1(\cdot)$). 
% Since the additional overhead of the data-dependent approach increases only the second and third term of $\epsilon_1(\cdot)$, only when the first term dominates, will the improvement from the data-dependent bound be significant enough to outweigh the incurred additional pDP losses.

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/ep1_datasets_ep23.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Comparison of the pDP losses with the additional overhead added.}
%   \label{fig:ep1_ep23_compare}
% \end{figure}


% \subsection{True pDP loss $\epsilon_1$ vs. released bound $\tilde{\epsilon_1}$}

% \label{exp:first}
% In this experiment we use a synthetic dataset, sampling $\theta \sim \mathcal{N}(0, 1)$, sampling $X \in \mathbb{R}^{n \times d}$ from the $d$-dimensional unit ball. $Y$ is then a deterministic function of $X$ and $\theta$ such that Pr[$Y = 1$] = \texttt{sigmoid}($X^T \theta) + E$ for noise matrix $E$. Figure ~\ref{fig:histograms} plots the pDP distributions for the true $\epsilon_1$ and its data-independent bound $\tilde{\epsilon}$ calculated according to Algorithm ~\ref{alg:privacy_report}, demonstrating both that the true \emph{ex-post} pDP loss is an order of magnitude improvement compared to the worst case DP bound $\epsilon$, and that the data-independent bound provides a good approximation to the true pDP loss.

% Generate random \theta of dimensionality d, X of dimensionality n by d, Y = X^T \theta + noise.


% dimension logistic
% generate data with "generate_data" function (describe)
% vary d = [1, ..50, 60] and calculate 1) max_i \epsilon_1(i) and \epsilon_1^P(i) using data-independent bound...same for best-case and median case

% true_release_comp
% kidney dataset?
% for varying levels of \epsilon, do objective perturbation as described in Theorem ? and calculate pDP distributions for the true and released values of \epsilon_1, using data-independent bounds

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/true_release_comp.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{pDP distributions for the true $\epsilon_1$ and its data-independent bound.}
%   \label{fig:histograms}
% \end{figure}

% \subsection{Dimension}

% We generate synthetic data as described in the previous experiment, this time varying $d \in [1, 5, 10, 20, 30, 40, 50, 60]$. We choose $\epsilon = 0.5$ as the DP bound and $\delta = 10^{-3}$, and set $\sigma, \lambda$ according to Theorem ~\ref{thm:alg1}. Figure ~\ref{fig:dimension} plots the true worst-, best- and median-case \emph{ex-post} pDP loss over all individuals $z$ against its data-independent counterpart (i.e., the worst-case pDP loss is calculated as $\max_{z \in D} \epsilon(\cdot, D_{\pm z})$ and the worst-case data-independent bound as $\max_{z \in D} \Tilde{\epsilon}(\cdot, z)$).

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/dimension_logistic.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{pDP losses across varying data dimensions.}
%   \label{fig:dimension}
% \end{figure}




==> Privately Publishable Per-instance Privacy/sections/experiments_original.tex <==
% !TEX root = ../main.tex

We evaluate our methods to release the pDP losses across a variety of datasets, using linear and logistic regression as case studies.

\textbf{Experimental Setup}\: Throughout, we set $\delta = 10^{-6}$ (failure probability of Algorithm ~\ref{alg:Alg1}, i.e. objective perturbation) and $\rho = 10^{-6}$ (failure probability of Algorithm \ref{alg:privacy_report} that releases a private upper bound on the pDP loss). Our choice of $\sigma$ depends on $\epsilon_1$ and follows the requirements for objective perturbation stated in Theorem \ref{thm:alg1} to achieve DP.  Unless otherwise specified, we set $\lambda$ as described in Algorithm \ref{alg:privacy_report}. We don't use any additional regularization, i.e. $r(\theta) = 0$. The noise parameters $\sigma_2, \sigma_3$ are each calibrated according to the analytic Gaussian mechanism of \citep{balle2018improving}, with an equal privacy budget allotted to each private release. In other words, Algorithm \ref{alg:Alg1} which releases $\hat{\theta}^P$ has a budget of $\epsilon_1$; Algorithm \ref{alg:privacy_report} which releases $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$ has a budget of $2\epsilon_1$; and therefore the combined privacy budget of objective perturbation and releasing the associated pDP losses is equal to $3 \epsilon_1$.

\textbf{Datasets}
%kidney, synthetic, credit, liver, wine
For experiments related to linear regression, we use the wine quality dataset \citep{Dua:2019} from the UCI Machine Learning Repository. We also evaluate our methods on synthetic data generated by sampling $x_i, \theta \sim \mathcal{N}(0, I_d)$ and normalizing each $x_i \in X$ so that $||x_i||_2 = 1$. The unperturbed response variable $Y \in \mathbb{R}^n$ is then determined as $Y = X \theta$ and rescaled so that each $y_i \in [0, 1]$.

We use three UCI datasets to test our methods on logistic regression: the credit card default dataset \citep{yeh2009comparisons}, the chronic kidney disease dataset and the liver disorders dataset \citep{Dua:2019}. In addition, we generate synthetic data by sampling  $x_i, \theta \sim \mathcal{N}(0, I_d)$ and determining each $y_i$ as
%\centerline{
$$y_i = \begin{cases} 
        1 & \text{ if } \texttt{sigmoid}(x_i^T\theta) > 0.5, \\ 
        0 & \text{ otherwise.} \end{cases}$$
        %}

\subsection{Stronger regularization does not worsen model utility}
% logistic regression
% explain lambda_inflate
% star denotes the actual inflation value (how many times larger \lambda_{adapt} is than \lambda_{obj})
% can see it has minimial effect on the 0-1 loss of the model
\begin{minipage}{.4\textwidth}
Algorithm ~\ref{alg:privacy_report} requires a larger $\lambda$ than suggested by Theorem $\ref{thm:alg1}$ in order to achieve a uniform multiplicative approximation of $\mu(\cdot)$.  
We investigate the effect of stronger regularization on the utility of a private logistic regression model applied to a synthetic dataset ($n = 1000, d = 50$), for several settings of $\epsilon_1$. Since each value of $\epsilon_1$ demands a different minimum value of $\lambda$ in order to achieve $(\epsilon_1, \delta)$-differential privacy, we compare via "$\lambda$-inflation": a measure of how many times larger we set $\lambda$ than its minimum value required to achieve the worst-case DP bound of objective perturbation.
\end{minipage}
\hspace{.2cm}\begin{minipage}{.6\textwidth}
\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/lambda_utility.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Utility of Obj-Pert with larger $\lambda$.}
  \label{fig:lambda_utility}
\end{figure}
\end{minipage}

  E.g., for logistic regression the objective perturbation mechanism requires $\lambda \geq \frac{1}{2\epsilon}$, and so in Figure ~\ref{fig:lambda_utility} a $\lambda$-inflation value of 10 means that we set $\lambda = \frac{5}{\epsilon}$. For each $\lambda$-inflate value $c$ , we run Algorithm \ref{alg:Alg1} with $\lambda = c \lambda_{\texttt{Obj-Pert}}$.  In particular, the star symbol marks the level of $\lambda$-inflation enforced by Algorithm ~\ref{alg:privacy_report}. The experimental results summarized in Figure ~\ref{fig:lambda_utility} show that the performance of the private logistic regression model (as measured by the 0-1 loss) remains roughly constant across varying scales of $\lambda$.


\subsection{Comparison of data-independent and data-dependent bounds}

Algorithm ~\ref{alg:privacy_report} presents two approaches to releasing a private upper bound of $\epsilon_1(\cdot)$, the pDP loss of releasing $\hat{\theta}^P$ from Algorithm ~\ref{alg:Alg1}. The data-independent approach bounds the pDP loss using only individual $z$'s own data as well as publicly-known parameters of the algorithm ($\rho, \sigma, \lambda$). The data-dependent approach privatizes the quantities $\mu(\cdot)$ and $g(\cdot) := \nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)$ that depend on the entire dataset. While the data-dependent approach can more accurately release $\overline{\epsilon_1^P}(\cdot)$, it suffers an additional privacy loss which could negate the savings of a more accurate bound on the pDP loss of Algorithm ~\ref{alg:Alg1}. It is therefore of interest to us to investigate the trade-offs of both approaches.

First, we run both the data-independent and -dependent variations of Algorithm ~\ref{alg:Alg1} with privacy parameters set to achieve $\epsilon_1 = \epsilon_2 = \epsilon_3 = 1$, as described in the experimental setup. Figure ~\ref{fig:ep1_compare} compares the distributions of the true pDP loss $\epsilon_1(\cdot)$ and its privately released upper bound $\overline{\epsilon_1^P}(\cdot)$ using both the data-independent and -dependent approaches. We see that for the same privacy budget $\epsilon_1 = 1$ allotted to Algorithm ~\ref{alg:Alg1} (indicated by the red line), the data-dependent upper bound is significantly tighter than the data-independent upper bound. However, Figure ~\ref{fig:ep1_compare} doesn't take into account the additional privacy loss incurred by using the data-dependent version of Algorithm ~\ref{alg:privacy_report}.

\begin{figure}[H]
  \centering
\includegraphics[width=\textwidth]{experiments/ep1_datasets.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Comparison of pDP losses and data-independent and -dependent upper bounds}
  \label{fig:ep1_compare}
\end{figure}

Figure ~\ref{fig:ep1_ep23_compare} includes the additional per-instance privacy loss of Algorithm ~\ref{alg:privacy_report} (for the data-independent version, we simply have $\epsilon_2(\cdot) = \epsilon_3(\cdot) = 0$). When considering the combined pDP loss of running Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report}, the data-independent bound is tighter. However, it is perhaps unfair of us to compose the \emph{ex-post} pDP loss of Algorithm ~\ref{alg:Alg1} with the \emph{ex-ante} pDP loss of Algorithm ~\ref{alg:privacy_report}, particularly given that the the \emph{ex-ante} pDP loss of Algorithm ~\ref{alg:privacy_report} has a necessary dependence on the order of $\sqrt{2\log(1/\delta)}$. In the appendix, we explore how to allocate the privacy budget between Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report} in order to achieve a more favorable trade-off between the data-independent and data-dependent approaches.

Based on our theory and experiments, our recommendation is to use data-independent bounds if $\lambda$ is large (the second or the third term dominates $\epsilon_1(\cdot)$). 
The data-dependent bound (and the adaptive algorithm presented in the appendix) may be preferred if $\lambda$ is small and the $-\log(1-\mu(\cdot))$ term dominates  the $\epsilon_1(\cdot)$). 
Since the additional overhead of the data-dependent approach increases only the second and third term of $\epsilon_1(\cdot)$, only when the first term dominates, will the improvement from the data-dependent bound be significant enough to outweigh the incurred additional pDP losses.

\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/ep1_datasets_ep23.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Comparison of the pDP losses with the additional overhead added.}
  \label{fig:ep1_ep23_compare}
\end{figure}


% \subsection{True pDP loss $\epsilon_1$ vs. released bound $\tilde{\epsilon_1}$}

% \label{exp:first}
% In this experiment we use a synthetic dataset, sampling $\theta \sim \mathcal{N}(0, 1)$, sampling $X \in \mathbb{R}^{n \times d}$ from the $d$-dimensional unit ball. $Y$ is then a deterministic function of $X$ and $\theta$ such that Pr[$Y = 1$] = \texttt{sigmoid}($X^T \theta) + E$ for noise matrix $E$. Figure ~\ref{fig:histograms} plots the pDP distributions for the true $\epsilon_1$ and its data-independent bound $\tilde{\epsilon}$ calculated according to Algorithm ~\ref{alg:privacy_report}, demonstrating both that the true \emph{ex-post} pDP loss is an order of magnitude improvement compared to the worst case DP bound $\epsilon$, and that the data-independent bound provides a good approximation to the true pDP loss.

% Generate random \theta of dimensionality d, X of dimensionality n by d, Y = X^T \theta + noise.


% dimension logistic
% generate data with "generate_data" function (describe)
% vary d = [1, ..50, 60] and calculate 1) max_i \epsilon_1(i) and \epsilon_1^P(i) using data-independent bound...same for best-case and median case

% true_release_comp
% kidney dataset?
% for varying levels of \epsilon, do objective perturbation as described in Theorem ? and calculate pDP distributions for the true and released values of \epsilon_1, using data-independent bounds

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/true_release_comp.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{pDP distributions for the true $\epsilon_1$ and its data-independent bound.}
%   \label{fig:histograms}
% \end{figure}

% \subsection{Dimension}

% We generate synthetic data as described in the previous experiment, this time varying $d \in [1, 5, 10, 20, 30, 40, 50, 60]$. We choose $\epsilon = 0.5$ as the DP bound and $\delta = 10^{-3}$, and set $\sigma, \lambda$ according to Theorem ~\ref{thm:alg1}. Figure ~\ref{fig:dimension} plots the true worst-, best- and median-case \emph{ex-post} pDP loss over all individuals $z$ against its data-independent counterpart (i.e., the worst-case pDP loss is calculated as $\max_{z \in D} \epsilon(\cdot, D_{\pm z})$ and the worst-case data-independent bound as $\max_{z \in D} \Tilde{\epsilon}(\cdot, z)$).

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/dimension_logistic.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{pDP losses across varying data dimensions.}
%   \label{fig:dimension}
% \end{figure}



==> Privately Publishable Per-instance Privacy/sections/introduction.tex <==
% !TEX root = ../main.tex

An explosion of data has fueled innovation in machine learning applications and demanded, in equal turn, privacy protection for the sensitive data with which machine learning practitioners train and evaluate models.

Differential privacy (DP) \citep{dwork2006calibrating, dwork2014algorithmic} has become a mainstay of privacy-preserving data analysis, replacing less robust privacy definitions such as \textit{k}-anonymity which fail to protect against sufficiently powerful de-anonymization attacks \citep{narayanan2008robust}. In contrast, DP offers provable privacy guarantees that are robust against an arbitrarily strong adversary.

The data curator could trivially protect against privacy loss by reporting a constant function, or by releasing only data-independent noise. The key challenge of DP is to release privatized output that retains utility to the data analyst.

A desired level of utility in a machine learning application might necessitate a high value of $\epsilon$, but the privacy guarantees degrade quickly past $\epsilon = 1$. \citep{triastcyn2020bayesian} construct an example whereby a differentially private algorithm with $\epsilon = 2$ allows an attacker to use a maximum-likelihood estimate to conclude with up to 88\% accuracy that an individual is in a dataset. For $\epsilon = 5$, the theoretical upper bound on the accuracy of an optimal attack is 99.3\%.

Moreover, practical applications of differential privacy commonly use large values of $\epsilon$. A study of Apple's deployment of differential privacy revealed that the overall daily privacy loss permitted by the system was as high as $\epsilon = 6$ for Mac OS 10.12.3 and $\epsilon = 14$ for iOS 10.1.1 \citep{tang2017privacy} -- offering only scant privacy protection!

Recent work \citep{yu2021large} has empirically justified large privacy parameters by conducting membership inference attacks to demonstrate that these seemingly tenuous privacy guarantees are actually much stronger in practice. These results are unsurprising from the perspective that DP gives a data-independent bound on the worst-case privacy loss which is likely to be a conservative estimate of the risk to a particular individual when a DP algorithm is applied to a particular input dataset.

\emph{Per-instance differential privacy} provides a theoretically sound alternative to the empirical approach for revealing the gap between the worst-case DP bound and the actual privacy loss in practice. The privacy loss to a particular individual relative to a fixed dataset might be orders of magnitude smaller than the worst-case bound guaranteed by standard DP. In this case, an algorithm meeting a desired level of utility but providing weak DP guarantees may, for the same level of utility, achieve drastically more favorable $\emph{per-instance}$ DP guarantees.

% also -- many machien learning applications are data-dependent
The remaining challenge is that the per-instance privacy loss is a function of the entire dataset; publishing it directly would negate the purpose of privately training a model in the first place! In this paper, we propose a methodology to privately release the per-instance privacy losses associated with private empirical risk minimization. Our contributions are as follows:
\begin{itemize}
    \item We introduce \emph{ex-post} per-instance differential privacy to provide a sharp characterization of the privacy loss to a particular individual that adapts to both the input dataset and the algorithm's output.
    \item We present a novel analysis of the \emph{ex-post} per-instance privacy losses incurred by the objective perturbation mechanism, demonstrating that these \emph{ex-post} pDP losses are orders of magnitude smaller than the worst-case guarantee of differential privacy.
    \item We propose a group of methods to privately and accurately release the \emph{ex-post} pDP losses. In the particular case of generalized linear models, we show that we can accurately publish the private \emph{ex-post} pDP losses using a dimension- and dataset-independent bound.
    \item One technical result of independent interest is a new DP mechanism that releases the Hessian matrix by adding a \emph{Gaussian Orthogonal Ensemble} matrix, which improves the classical ``AnalyzeGauss'' \citep{dwork2014analyze} by roughly a constant factor of $2$.
\end{itemize}



% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=\textwidth]{illustration.pdf}
% 	\vspace{-2em}
% 	\caption{An illustration of the proposed new model for releasing a comprehensive privacy report.}\label{fig:illus}
% \end{figure*}
% (adversary-specific -- but the definition is mostly a convenience to formalize the intuition that a target individual's privacy can be threatened only by the observable output of a mechanism.)


==> Privately Publishable Per-instance Privacy/subsections/differential_privacy.tex <==
% !TEX root = ../main.tex

    Let $\mathcal{Z}$ denote the data domain, and $\mathcal{R}$ the set of all possible outcomes of algorithm $\mathcal{A}$. Fix $\epsilon, \delta \geq 0$.
    \begin{defn} (Differential privacy)  \label{def:dp}
        A randomized algorithm $\mathcal{A}: \mathcal{Z}^* \rightarrow \mathcal{R}$ satisfies $(\epsilon, \delta)$-DP if for all datasets $D \in \mathcal{Z}^{*}$ and data points $z \in \mathcal{Z}$, and for all measurable sets $S \subset \mathcal{R}$, 
        \begin{align*}
            &\text{Pr}\big[\mathcal{A}(D) \in S\big] \leq e^{\epsilon}\text{Pr}\big[\mathcal{A}(D_{\pm z}) \in S\big] + \delta.
        \end{align*}
    \end{defn}
    
    Differential privacy guarantees that the presence or absence of any particular data record has little impact on the output distribution of a randomized algorithm. In this paper we use the "add/remove" notion of DP, by which we construct neighboring dataset $D_{\pm z}$ by adding or removing an individual $z$ from dataset $D$. %, rather than the "replace one" version of DP which constructs $D'$ by removing individual $i$ and adding individual $i' \neq i$. 
    
    DP is powerful and universal in that its guarantee applies to any $D, z$ and set of output events.  However, there are often situations where the privacy losses of $\mathcal{A}$ vary drastically depending on its input data, and the  privacy loss bound $\epsilon$ (protecting even the worst-case pair of neighboring datasets) may not be informative of the privacy loss incurred to individuals when the input to $\mathcal{A}$ is typical.  This motivated \citep{wang2019per} to consider a per-instance version of the DP definition. 
        \begin{defn} (Per-instance differential privacy)  \label{def:pdp}
    	A randomized algorithm $\mathcal{A}: \mathcal{Z}^* \rightarrow \mathcal{R}$ satisfies $\big(\epsilon(D, D_{\pm z}), \delta\big)$-pDP if for dataset $D$ and data point $z$, and for all measurable sets $S \subset \mathcal{R}$, 
    	\begin{align*}
    	&\text{Pr}\big[\mathcal{A}(D) \in S\big] \leq e^{\epsilon}\text{Pr}\big[\mathcal{A}(D_{\pm z}) \in S\big] + \delta,\\
    	&\text{Pr}\big[\mathcal{A}(D_{\pm z}) \in S\big] \leq e^{\epsilon}\text{Pr}\big[\mathcal{A}(D) \in S\big] + \delta.
    	\end{align*}
    \end{defn}
The pDP definition can be viewed as using a function $\epsilon(D,D_{\pm z})$ that more precisely describes the privacy guarantee in protecting a fixed data point $z$ when $\mathcal{A}$ is applied to dataset $D$. 

    %We argue that the "add/remove" definition of neighboring datasets gives a more general form of differential privacy than the "replace one" version, since we can always recover the "replace one" version by twice applying the "add/remove" version to remove individual $i$ and then adding individual $i'$.
    
%
%    \begin{defn} (\textit{Ex-post} per-instance differential privacy)
%        A randomized algorithm $\mathcal{A}$ satisfies $(\epsilon(\mathcaldot), \delta)$-\textit{ex-post} per-instance differential privacy for an individual $z$ and a fixed dataset $D$ if given an outcome $o = \mathcal{A}(D)$, it holds that
%        \begin{align*}
%            &\text{Pr}\big[\mathcal{A}(D) = o \big] \leq e^{\epsilon}\text{Pr}\big[\mathcal{A}(D_{\pm z}) = o\big] + \delta. \\
%            &\text{Pr}\big[\mathcal{A}(D_{\pm z})= o\big] \leq e^{\epsilon}\text{Pr}(\mathcal{A}(D)= o\big] + \delta.
%        \end{align*}
%    \end{defn}
%    

% Both DP and pDP are about the \emph{ex ante} properties of the mechanism $\mathcalA$ before it is applied. Following the definition of \emph{ex post} DP pioneered by \mathcalitep{ligett2017accuracy}, 

As it turns out, it is most convenient for us to work with an even more  \emph{instance-specific} description of the privacy loss that is further parameterized by the realized output of $\mathcal{A}$ \emph{ex-post} --- after the random coins of $\mathcal{A}$ are flipped and the outcome released.
%It turns out that it is more convenient for us to work with an even more adaptive notion 
\begin{defn} (\textit{Ex-post} per-instance differential privacy)\label{def:expost_pdp}
	A randomized algorithm $\mathcal{A}$ satisfies $\epsilon(\cdot)$-\emph{ex-post} per-instance differential privacy for an individual $z$ and a fixed dataset $D$ at an outcome $o\in \mathrm{Range}(\mathcal{A})$ if 
	$$
	\left|\log\left(\frac{\text{Pr}\big[\mathcal{A}(D) = o \big]}{\text{Pr}\big[\mathcal{A}(D_{\pm z})= o\big]}\right)\right| \leq \epsilon(o,D,D_{\pm z}). 
	$$ 
\end{defn}
% discuss a bit more...
This definition generalizes the \emph{ex-post} DP definition \citep{ligett2017accuracy} (introduced for a different purpose) to a \emph{per-instance} version that depends on a given pair of neighboring datasets.
%The ex-post DP definition \mathcalite{ligett2017accuracy} was designed to analyze algorithms whose privacy guarantees aren't fixed but rather depend on properties of the computation. 
The above quantity is essentially the absolute value of the log-odds ratio, used extensively in hypothesis testing. Intuitively, the $\emph{ex-post}$ per-instance privacy loss $\epsilon(o, D, D_{\pm z})$ describes how confidently an attacker could infer, given the output of algorithm $\mathcal{A}$, whether or not individual $z$ is in dataset $D$.
% We make three important remarks.  First, the definition is essentially the absolute value of the log-odds ratio, used extensively in hypothesis testing.  Second, if $\mathcalA$ satisfies DP, then the output $o$ is privately released and thus there is no ``catch'' in using $o$ for subsequent computation thanks to the information-processing inequality of DP.  Third, \emph{Ex-post} pDP is also related to the concept of privacy loss random variable, which considers $\log(p(o) / q(o))$ for $o\sim \mathcalA(D)$ ($p,q$ are shorthands for the density function of $\mathcalA(D)$ and $\mathcalA(D_{\pm z})$), and had been a central object in the composition of DP mechanisms, and in modern DP techniques such as concentrated DP, Renyi DP and privacy profile \mathcalitep[see, e.g.,][for a good review]{mironov2017renyi,balle2018privacy}. 

%This perspective is convenient for our analysis of Algorithm~\ref{alg:Alg1}, whose privacy parameters are a function of the data. Since we are analyzing the per-instance privacy cost of \emph{releasing} $\hat{\theta}^P$, it makes perfect sense to condition the pDP loss on the privatized output of the computation.

Despite (or perhaps because of) its precise accounting for privacy, \emph{ex-post} pDP could reveal sensitive information about the dataset, as the following example explicitly illustrates.
\begin{example}[The privacy risk of exposing \emph{ex-post} pDP]\label{ex:privacy_risk}
Consider a standard Gaussian mechanism $\mathcal{A}$ that adds noise to a counting query $Q$ applied to dataset $D$, i.e. $\mathcal{A}(D) = Q(D) + \mathcal{N}(0, \sigma^2)$. $Q$ has global sensitivity $\Delta_Q = 1$.  We will show that an attacker, knowing only the output $o$ of algorithm $\mathcal{A}$, her \emph{ex-post} pDP loss and that her individual data is not contained in dataset $D$, can conclusively uncover the sensitive quantity $Q(D)$ protected by algorithm $\mathcal{A}$.

Following the proof of Theorem \ref{pdp_gaussian}, the \emph{ex-post} pDP can be directly calculated as 
\begin{align*}\epsilon(o, D,D_{\pm z}) = \frac{|Q(D)-Q(D_{\pm z})||2o - Q(D) -  Q(D_{\pm z})| }{2\sigma^2}.\end{align*}

Enter attacker $z$, who has auxiliary information: she knows that her own individual data is not contained in $D$. After algorithm $\mathcal{A}$ is applied to $D$, attacker $z$ receives output $o = 1$ and is informed of her \emph{ex-post} pDP $\epsilon(o, D,D_{+z})$. Since $Q(D_{+z}) = Q(D) + 1$ is known, attacker $z$ can solve for $Q(D)$ and obtain $Q(D) = o - 0.5 \pm \sigma^2 \epsilon(o, D,D_{+z})$. With probability $1$, only one of the two possibilities is an integer\footnote{Take $Q(D) = 0$ and $o = 0.1$ as an example, the two possibilities are $0$ and $-0.8$.}. Therefore, exposing \emph{ex-post} pDP in this case completely reveals $Q(D)$.
% 	Consider a standard Gaussian mechanism, applied to a counting query $Q$ on $D$ (with global sensitivity $1$).  Let $o\sim \mathcalN(Q(D), \sigma^2)$, then it is easy to calculate the \emph{ex-post} pDP to be $\epsilon(o, D,D') = \frac{|Q(D)-Q(D')||2o - Q(D) -  Q(D')| }{2\sigma^2}$.
% Let the attacker $z$ be the one who knows that herself is not in $D$, her value to the counting query is $1$ and she was informed about her \textit{ex-post} pDP  $\epsilon(o, D,D_{+z})$.  Note that $Q(D_{+z}) = Q(D) + 1$ is known thus, one can solve for $Q(D)$ and obtain $Q(D) = o - 0.5 \pm \sigma^2 \epsilon(o, D,D_{+z})$. With probability $1$, only one of the two possibilities is an integer\footnote{Take $Q(D) = 0$ and $o = 0.1$ as an example, the two possibilities are $0$ and $-0.8$.}, therefore exposing \emph{ex-post} pDP in this case completely reveals $Q(D)$.
\end{example}
% A more general pDP analysis of the Gaussian mechanism (when $Q$ is an arbitrary function of the data) is provided in Section~\ref{sec:}, which we will use later for privately publishing the \emph{ex-post} pDP losses.


\noindent\textbf{Problem statement.} The lesson of Example \ref{ex:privacy_risk} is that we cannot directly reveal the \emph{ex-post} pDP losses without potentially nullifying the algorithm's privacy benefits. How, then, can we privately and accurately publish the \emph{ex-post} pDP losses?

The goal of this paper is to develop an algorithm that publishes a \emph{function} $\tilde{\epsilon}: \mathcal{Z} \rightarrow \mathbb{R}$ whose output estimates the \emph{ex-post} pDP loss to an individual $z$ of releasing the output $\hat{\theta}^P$ from the objective perturbation mechanism. Any individual (not just those whose data is contained in the dataset) can plug her own data $z$ into this function in order to receive a high-probability bound on her \emph{ex-post} pDP loss which does not depend directly on any sensitive data except her own.

This requirement offers the same type of privacy protection as joint differential privacy \citep{kearns2014mechanism}, which relaxes the standard DP definition by allowing an algorithm's output to individual $z$ to be sensitive only in her own private data.  Our notion of privacy is slightly more general in that it holds for individuals both in and out of the dataset. The difference lies in how the algorithm's output space is defined; whereas a joint DP algorithm produces a fixed-length tuple partitioning the output to each individual in the dataset, our algorithm outputs a function whose domain includes any data point $z \in \mathcal{Z}$. As a result, our methods are robust against collusion by arbitrary coalitions of adversaries, allowing repeated queries by any group of individuals without invalidating the privacy guarantees promised by the pDP losses.
% tuple {}_{-i} vs 
% change the output space
% can be in or out of the dataset;
% \noindent\textbf{Problem statement.} The goal of this paper is to develop a DP mechanism $\mathcalB$ that publish the \emph{ex-post} pDP for $\mathcalA$ as well as the  \emph{ex-post} pDP for $\mathcalB$ itself. The output should be a function such that any individual $z$ could query for approximately how much privacy loss she incurs, while having the ease of mind that other people who receive the same information  collectively will not invalidate the \emph{ex-post} pDP bound that $z$ just saw.
% % give definition and intuitive explanation
% % indistinghuisble outcome between adjacent datasets

% Our requirement for $\mathcalB$ is related to but different from a joint-differentially private mechanism $\tilde{B}$. The difference is that  $\mathcalB$ outputs $\epsilon(o,D,D_{\pm z})$ a function $\tilde{\epsilon}(\mathcaldot)$ of $z$ under the standard DP definition where $z$ could be any individual regardless of whether $z$ in the dataset $D$ or not ; while the output of $\tilde{B}$ is the tuple of \textit{ex-post} pDP losses  $\epsilon(o,D,D_{-z_j})$ for all $z_j \in D$, and it is different from DP because the adversary is defined with respect to each individual $z_i$ who observes $\epsilon(o,D,D_{-z_j})$ for all $z_j\in D$ except when $j=i$. 



==> Privately Publishable Per-instance Privacy/subsections/notations.tex <==
% !TEX root = ../main.tex

We write the output of a randomized algorithm $\mathcal{A}$ as $\mathcal{A}(\cdot)$, and for continuous distributions we take $\text{Pr}[\mathcal{A}(D) = o]$ to be the value of the probability density function at output $o$.

We will let $z\in \cZ$ refer to both an individual and their data; for example, individual $z$ holds data $z=(x, y)$ in a supervised learning problem. We take $\cZ^*=\cup_{n=0}^\infty \cZ^n$ to be the space of datasets with an unspecified number of data points. $D_{\pm z} \in \mathcal{Z}^*$ denotes the fixed dataset $D = \{z_1,\ldots,z_n\} \in \mathcal{Z}^*$ with the data point $z$ removed from $D$ if $z \in D$, 
%and the point $z$ 
or added to $D$ if $z \notin D$. 
In our mathematical expressions, we use "$\pm$" to mean "add if $z \notin D$, subtract otherwise". Similarly. "$\mp$" means "subtract if $z \notin D$, add otherwise".

We distinguish between $\epsilon$ as fixed input to a DP algorithm, and $\epsilon(\cdot)$ as a function parameterized according to a particular DP relaxation ---  e.g., $\epsilon(o, D, D_{\pm z})$ means the \textit{ex-post} per-instance privacy loss conditioned on output $o$, dataset $D$, and data point $z$.


==> Privately Publishable Per-instance Privacy/subsections/objective_perturbation.tex <==
% !TEX root = ../main.tex

    The objective perturbation algorithm solves
    \begin{align}
        \hat{\theta}^P &= \argmin\limits_{\theta \in \Theta} L(\theta ; D) + r(\theta) + \frac{\lambda}{2}||\theta||_2^2 + b^T\theta, \label{op}
    \end{align}
    where $b \sim \mathcal{N}(0, \sigma^2I_d)$ and parameters $\sigma, \lambda$ are chosen according to a desired $(\epsilon, \delta)$-DP guarantee.
% the choice of $\sigma$ depends on the privacy budget $\epsilon$, the failure probability $\delta$, smoothness parameter $\beta$, and an upper bound $\rho_{\text{max}}$ on the eigenvalues of $\nabla^2 \ell(x^T \theta; y)$ for all $(x, y)$ and $\theta \in \Theta$. The regularization parameter $\lambda$ must also be chosen so that the objective function \ref{obj_j} is strongly convex.
    \begin{algorithm}[H]
        \caption{Release $\hat{\theta}^P$ via \texttt{Obj-Pert} \citep{kifer2012private}}
        \label{alg:Alg1}
        \begin{algorithmic}
            \STATE{{\bfseries Input:} Dataset $D$, noise parameter $\sigma$, regularization parameter $\lambda$, loss function $L(\theta; D) = \sum_i \ell(\theta; z_i)$, convex and twice-differentiable regularizer $r(\theta)$, convex set $\Theta$.}
            \STATE{{\bfseries Output:} $\hat{\theta}^P$, the minimizer of the perturbed objective.}
           \STATE{Draw noise vector $b \sim \mathcal{N}(0, \sigma^2I)$.}
           \STATE{Compute $\hat{\theta}^P$ according to (\ref{op}).}
        \end{algorithmic}
    \end{algorithm}
    
    \begin{theorem}[Privacy guarantees of Algorithm~\ref{alg:Alg1} \citep{kifer2012private}]
        \label{thm:alg1}
        Consider dataset $D = \{z_i\}_{i = 1}^n$; loss function $L(\theta; D) = \sum_i \ell(\theta; z_i)$; convex regularizer $r(\theta)$; and convex domain $\Theta$. Assume that $\nabla^2 \ell(\theta; z_i) \prec \beta I_d$ and $||\nabla \ell(\theta; z_i)||_2 \leq \xi$ for all $z_i \in \mathcal{X} \times \mathcal{Y}$ and for all $\theta \in \Theta$.
        % Let $\beta$ be an upper bound on the eigenvalues of the Hessian $\nabla^2 \ell(\theta; z_i)$, for all $z_i \in \mathcal{X} \times \mathcal{Y}$ and for all $\theta \in \Theta$. Let $\ell(\cdot)$ have a bounded gradient such that $||\nabla \ell(\theta; z_i)||_2 \leq \xi$ for all $z_i \in \mathcal{X} \times \mathcal{Y}$ and for all $\theta \in \Theta$.
        For $\lambda \geq 2\beta/\epsilon_1$ and $\sigma = \xi^2(8 \log (2/\delta) + 4\epsilon_1)/\epsilon_1^2$, Algorithm~\ref{alg:Alg1} satisfies $(\epsilon_1, \delta)$-differential privacy.
    \end{theorem}
    
    The privacy guarantees stated in Theorem \ref{thm:alg1} apply even when $\theta$ is constrained to a closed convex set, but for ease of our per-instance privacy analysis we will require $\Theta = \mathbb{R}^d$ from this point on.
    % Algorithm ~\ref{alg:Alg1} is an abridged version of \citep{kifer2012private}'s \texttt{Obj-Pert} mechanism which can achieve pure $\epsilon$-DP by adding Gamma noise instead of Gaussian. \citep{kifer2012private}'s algorithm also extends \texttt{Obj-Pert} to handle convex constraints, but for ease of our privacy analysis we will require $\Theta = \mathbb{R}^d$ from this point on.
    
% Our simplified version of $\texttt{Obj-Pert}$ differs in a couple of ways from the algorithm presented in \cite{kifer2012private}. We analyze only the Gaussian noise case, thereby permitting a small failure probability $\delta_1$ and relaxing our privacy definition to approximate pDP.

%  In other words, for sufficiently large $\lambda$, the minimizer of an objective function that is $\lambda$-strongly convex will be insensitive to any particular data point.

% Though the $(\epsilon, \delta)$-differential privacy guarantees of Algorithm~\ref{alg:Alg1} apply to any convex objective function, we decide to focus on generalized linear models for a more transparent exposition. %Our techniques are applicable to the more general settings 
% %our pDP analysis applies primarily to generalized linear problems. 
% For the remainder of the paper we will tighten our assumptions on the problem setting and require that $L(\theta; D)$ be a linear loss function with the structure described in Section~\ref{problem_setting}.
% In the appendix we include pDP analysis of alg 1 for a general convex function

% note that alg 1 guarantees apply to any generalized convex loss function, but for our pDP analysis we will study only generalized linear functions

% The objective perturbation mechanism adds enough regularization to make the objective function strongly convex, also requires smoothness. operates under the intuition that when the Hessian of the objective function is well-conditioned, a small perturbation to it will not much affect the optimization. so achieves strong utility guarantees while masking privacy
% regularization and noise parameters depend on...
%

% In the interest of clarity, Algorithm~\ref{alg:Alg1} obfuscates several important details of $\texttt{Obj-Pert}$ --- namely, the choice of $\sigma$ and $\lambda$. Leaving the details to \cite{kifer2012private}, we remark that in order to achieve $(\epsilon_1, \delta_1)$-DP, the noise parameter $\sigma$ should be calibrated according to privacy parameters $\epsilon_1$ and $\delta_1$, in addition to properties of the gradient and Hessian of $\ell(\cdot)$. Similarly, the regularization parameter $\lambda$ should be chosen as a function of $\epsilon_1$ and the maximum eigenvalue of $\nabla^2 \ell(\cdot)$; this will ensure that the objective function is well-conditioned and therefore robust to small perturbations. In other words, for sufficiently large $\lambda$, the minimizer of an objective function that is $\lambda$-strongly convex will not depend too much on any particular data point.


%ex-post analysis inherits the guarantees against the worst-case (\epsilon, \delta)of Obj-Pert...but also adapts to the data to provide a stronger bound.


==> Privately Publishable Per-instance Privacy/subsections/overflow_algorithms_and_proofs.tex <==
% !TEX root = ../main.tex

        \begin{algorithm}[H]
        \caption{Dataset-dependent privacy report for \texttt{Obj-Pert} on GLMs}
        \label{alg:dataset_dependent_report}
        \begin{algorithmic}
            \STATE {\bfseries Input:} $\hat{\theta}^p$ from \texttt{Obj-Pert}, noise parameter $\sigma_1,\sigma_2,\sigma_3$; regularization parameter $\lambda$; Hessian $H := \sum_i\nabla^2\ell_i(\hat{\theta}^p) + \lambda I_d$.
            \STATE {\bfseries Output:} Reporting function $\tilde{\epsilon}: (x,y),\delta \rightarrow \R_+^2$
            \STATE Privately release $\hat{H}^p$ by Algorithm~\ref{alg:release_H} with parameter $\sigma_2$. 
             \STATE Sets $\epsilon_2(\cdot))$  according to Theorem~\ref{thm:pdp_of_H_lambda_min}.
            \STATE Set $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$.
            $\tau$ is on the order of $O(\sqrt{d}(1 + \log(C/\rho)^{3/2}))$ by Lemma~\ref{lem:lambda_GOE}.
            \STATE \IF{$\lambda \geq  2 \tau \sigma_2$}
            \STATE Set $\overline{\mu^p}(x) = \min\{\frac{3}{2}x^T [\hat{H}^p]^{-1} x,\frac{\|x\|^2}{\lambda}\}$
            \STATE Set $\epsilon_3(\cdot)\equiv 0$ 
            \ELSE
            \STATE Privately release $\hat{\lambda}_{\min}^p = \lambda_{\min} + \cN(0,\sigma_3^2)$.
              \STATE Sets $\epsilon_3(\cdot))$  according to Theorem~\ref{thm:pdp_of_H_lambda_min}.
            \STATE \IF{$\underline{\hat{\lambda}_{\min}^p}:=\hat{\lambda}_{\min}^p - \sigma_3 F_{\cN(0,1)}^{-1}(1-\rho/2)\geq  2 \tau\sigma_2$}
            \STATE Set $\overline{\mu^p}(x) = \min\{\frac{3}{2} x^T [\hat{H}^p]^{-1} x,\frac{\|x\|^2}{\max\{\lambda, \underline{\hat{\lambda}_{\min}^p}\}}\}$
            \ELSE 
            \STATE Set $\overline{\mu^p}(x) = \min\{\frac{\lambda + \tau \sigma_2}{\lambda } x^T (\hat{H}^p +  \tau \sigma_2 I_d)^{-1} x,\frac{\|x\|^2}{\max\{\lambda, \underline{\hat{\lambda}_{\min}^p}\}}\}.$
            \ENDIF 
            \ENDIF
            \STATE Set $\overline{\epsilon_1^p}(z):= \max\left\{
            \left|-\log \big(1 \pm f''(z,\hat{\theta}^p)\overline{\mu^p}(x) \big) + \frac{|f'(z,\hat{\theta}^p)|^2||x||^2}{2\sigma_1^2}  \pm  \frac{|f'(z,\hat{\theta}^p)|||x|| F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2})}{\sigma_1} \right|\right\}$.
            \yw{The maximum above is for the two possiblities, $\pm$.}
            \STATE Set $\tilde{\epsilon}_1(\cdot) = (\overline{\epsilon_1^p}(\cdot), \epsilon_2(\cdot) + \epsilon_3(\cdot))$
            \yw{Let's drop the lower bound and focus on separately reporting the released ex post-PDP parameter and then report the addtional overhead separately.}
            \yw{We could also simplify this algorithm so we only talk about the setting with sufficiently large $\lambda$.  Then we can say that we also propose a more adaptive algorithm that allows us to release valid bounds for all choices of $\lambda >0$ and adapt to well-conditioned $H$. Say that it is more tedious thus we include it only in the appendix.  Notice that the theorems that I stated are all about the case when $\lambda$ is large.}
            \vspace*{1mm}
        \end{algorithmic}
    \end{algorithm}
    
       Note that the pDP functions of the reporting algorithm $\epsilon_2(\cdot), \epsilon_3(\cdot)$ does not depend on the dataset, and thus is not required to be separately released.
    
       \begin{proposition}[Uniform privacy report]
    With probability $1-2\rho$,  \emph{simultaneously} for all $n$ users in the dataset, $\epsilon_1(z,\hat{\theta}^p) \leq \overline{\epsilon_1}^P(z,\hat{\theta}^p) \leq 12 \sqrt{\log n} \epsilon_1(z,\hat{\theta}^p)$
    
    If we, instead, use $\frac{|f'(z,\hat{\theta}^p)|\|x\|_1\sqrt{2\log(2d/\rho)}}{\sigma_1} $ to replace the third-term in $\overline{\epsilon^p}_1$, then with probability $1-2\rho$, \emph{simultaneously} for all $x\in\cX$, the ex post pDP report $\overline{\epsilon^p}_1$ satisfies that
    $$\epsilon_1(z,\hat{\theta}^p) \leq \overline{\epsilon^p}_1(z,\hat{\theta}^p) \leq 12 \sqrt{d\log d}\epsilon_1(z,\hat{\theta}^p).$$ 
        % \item With probability $1-\rho$, \emph{uniformly} For all $(x,y)\in\R^d\times \mathcal{Y},$ the \emph{ex post} pDP loss 
        % $\epsilon(z,\hat{\theta}^p) \leq $
    \end{proposition}
    \begin{proof}
    We note that the approximation of $\mu_x$ is uniform for all $x$. It remains to consider a uniform bound for the third term over the randomness of ObjPert. The first statement follows by taking union bound. And the second result is achieved by Holder's inequality,  the concentration of max of iid Gaussian, and that $\|x\|_1\leq \sqrt{d}\|x\|_2$. 
    \end{proof}
    
     \begin{proposition}[Uniform multiplicative approximation of a regularized estimator]\label{prop:utility_H_regularized}
 Let $\hat{H}^P$ be constructed through Algorithm~\ref{alg:release_H} with parameter $\sigma_2$ and let $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$. Then with  probability $1-\rho$, for all $x\in \R^d$
     $$ x^T(\hat{H}^P + \tau \sigma_2 I_d)^{-1}x \leq \mu(x) \leq \frac{\lambda + 2\tau\sigma_2}{\lambda} x^T(\hat{H}^P + \tau\sigma_2 I_d)^{-1}x. $$
 \end{proposition}
 \begin{proof}
 We choose $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$. With probability $1-\rho/2$, the largest eigenvalue is smaller than $\tau$.
 Similarly, by symmetry, with probability $1-\rho/2$, the smallest eigenvalue is larger than $-\tau$.
 By a union bound,  we have that with probability $1-\rho$
  $\|Z\|_2\prec \tau,$ i.e., $-\tau I_d \prec Z\prec \tau I_d$.
\begin{align*}
H&\prec H + Z + \tau \sigma_2 I_d \prec H + 2\tau \sigma_2 I = \nabla^2 L(\hat{\theta}^P) + \lambda I_d + 2\tau\sigma_2 I_d \\
&\prec \frac{\lambda + 2\tau\sigma_2}{\lambda}(\nabla^2 L(\hat{\theta}^P) + \lambda I_d) = \frac{\lambda + 2\tau\sigma_2}{\lambda} H.
\end{align*} 
Take inverse on both sides, we get
$$
\frac{\lambda}{\lambda + 2\tau\sigma_2}H^{-1} \prec (\hat{H}^P + \tau \sigma_2 I_d)^{-1} \prec H^{-1}.
$$
Thus for all $x\in \R^d$,
$x^T(\hat{H}^P + \tau \sigma_2 I_d)^{-1}x \leq x^T H^{-1}x \leq \frac{\lambda + 2\tau \sigma_2}{\lambda} x^T(\hat{H}^P + \tau \sigma_2 I_d)^{-1}x.$
\end{proof}
 

The AnalyzeGauss algorithm however uses a slightly different Gaussian random matrix to privately release the upper-triangular part of $H$ with the standard Gaussian mechanism.
\begin{proposition}[Largest eigenvalue of the noise matrix of AnalyzeGauss]\label{lem:spectral_norm_analyzgauss}
Let $A$ be a symmetric Gaussian random matrix with iid entries drawn from $\cN(0,\sigma^2)$ on the upper triangular part of the matrix, then there exists a universal constant $C'$ such that with probability $1-\delta$
$$
\|A\|_2  \leq \sigma \sqrt{d}(3\sqrt{2} +C'(\log(\max\{2d,2C\}/\delta))^{2/3}.
$$
\end{proposition}
\begin{proof}
Let us construct 
$\tilde{A}= A + D $
where $D$ is the diagonal matrix where $D_{ii} = A_{ii} (\sqrt{2}-1)$.  Clearly, $\tilde{A}$ is a Gaussian orthogonal ensemble. Thus by Lemma~\ref{lem:max_of_subgaussian}, Lemma~\ref{lem:lambda_GOE} and the triangular inequality
$$
\|A\|_2 \leq \|\tilde{A}\|_2 + \|D\|_2 \leq \sqrt{2}\left(2 + \big(\frac{(\log(2C/\delta))}{c d}\big)^{2/3}\right) \sqrt{d\sigma^2} + \sigma (\sqrt{2}-1)\sqrt{2\log (2d/\delta)}.
$$
To get the desired result, we can take $\frac{\log(2C/\delta)}{cd} \leq \frac{\log(2C/\delta)}{c}$ (since $d\geq 1$) and that $\sqrt{x} \leq 1 + (x)^{2/3}$ for all $x>0$. $C'$ can be taken as $c^{-2/3}+(2-\sqrt{2})$. 
\end{proof}

\begin{remark}
Instead of ``analyze-gauss'' noise, it is arguably more natural to add a GOE noise where the diagonal elements receive a variance that is twice as large. This is because the sensitivity of the upper-triangular part of the matrix $H$ is naturally measured in terms of an $A$-norm where $A\in \R^{(\frac{d^2}{2}+d/2)\times (\frac{d^2}{2}+d/2)}$ is a diagonal matrix with all coordinates corresponding to the off-diagonal elements $H$ being $2$ and those cooresponding to the diagonal elements of $H$ being $1$. 
Let the perturbation (due to adding or removing one data point) being $xx^T$ and let $\Delta_x\in \R^{\frac{d^2}{2}+d/2}$ denotes the vectorized version of the upper triangular region of $xx^T$, then it is clear that $\|\Delta_x\|_A =  \|x\|^2$.
The corresponding multi-variate Gaussian mechanism add noises with covariance matrix $A^{-1}$, which involves adding twice as large a noise to the diagonal elements, i.e., the noise is a GOE random matrix! 
\end{remark}



\section{New method for privately releasing leverage scores}

% The new algorithm releases $H$ by a Gaussian mechanism.
% $$
% \hat{H}^p = H + Z
% $$
% where $Z$ is a symmetric Gaussian noise.


    \begin{algorithm}[H]
        \caption{ Release $H$ (a natural variant of ``Analyze-Gauss'') }
        \label{alg:release_H}
        \begin{algorithmic}
            \STATE{{\bfseries Input:} Dataset $D$, noise parameter $\sigma_2$, $H  = \sum_{i=1}^n \nabla^2\ell(z_i, \hat{\theta}^P) + \lambda I_d$.}
            \STATE{{\bfseries Output:} $\hat{H}^P$.}
           \STATE{Draw a  Gaussian random matrix $Z\in \R^{d\times d}$ with $Z_{i,j}\sim \cN(0,\sigma_2^2)$ independently.}
           \STATE{Output $\hat{H}^P = H + \frac{1}{\sqrt{2}}(Z + Z^T)$.}
        \end{algorithmic}
    \end{algorithm}
    
    \begin{algorithm}[H]
                        \caption{ Releasing the smallest eigenvalue of $H$ }                \label{alg:lambda_min}
        \begin{algorithmic}
            \STATE{{\bfseries Input:} Dataset $D$, noise parameter $\sigma_3$, $\lambda_{\min}$ denoting the smallest eigenvalue of $H$.}%  = \sum_{i=1}^n \nabla^2\ell(z_i, \hat{\theta}^P) + \lambda I_d$.}
            \STATE{{\bfseries Output:} $\hat{\lambda}_{\min}^P$.}
           \STATE{Output $\hat{\lambda}_{\min}^P = \lambda_{\min} + \cN(0,\sigma_3^2)$ .}
        \end{algorithmic}
    \end{algorithm}

\begin{theorem}\label{thm:pdp_of_H_lambda_min}
    Algorithm~\ref{alg:release_H} satisfies pDP with 
    $$
    \epsilon_2(z,\delta) = \frac{(f^{''}(x,\hat{\theta}^p))^2\|x\|^4}{4\sigma_2^2} +  \frac{f^{''}(x,\hat{\theta}^p)\|x\|^2\sqrt{\log(1/\delta)}}{\sigma_2},
    $$
    and $\hat{H}^p$ satisfies ex post pDP of the same $\epsilon$ with probability $1-2\delta$.
    
    Algorithm~\ref{alg:lambda_min} satisfies pDP with 
    $$
    \epsilon_3(z,\delta) = \frac{(f^{''}(x,\hat{\theta}^p))^2\|x\|^4}{2\sigma_3^2} +  \frac{f^{''}(x,\hat{\theta}^p)\|x\|^2\sqrt{2\log(1/\delta)}}{\sigma_3},
    $$
\end{theorem}
\begin{proof}
Algorithm~\ref{alg:release_H} is equivalent to releasing the vector 
$
[f_1, f_2]
$
using a standard Gaussian mechanism with $\cN(0,\sigma_2^2 I_{\frac{d^2}{2}+d/2})$, where $f_1\in\R^d$ is the diagonal of $H/\sqrt{2}$ and $f_2\in\R^{(d^2-d)/2}$ is the vectorized  the strict upper triangular part of $H$.

The per-instance L2-sensivitiy of $[f_1,f_2]$ is 
\begin{align*}
\|\Delta_x\|_2 &= f''(z,\hat{\theta}^p)\sqrt{\sum_{1\leq i<j\leq d}x_i^2x_j^2 + \sum_{k=1^d} x_{k,k}^4 (1/\sqrt{2})^2} \\
&= f''(z,\hat{\theta}^p)\sqrt{\frac{1}{2}\sum_{1\leq i,j\leq d}( x_i^2x_j^2 + \sum_{k=1^d} x_{k,k}^4} \\
&= \frac{f''(z,\hat{\theta}^p)}{\sqrt{2}}\|xx^T\|_F= \frac{f''(z,\hat{\theta}^p)}{\sqrt{2}}\|x\|_2^2.
\end{align*}
The result then follows from an application of the pDP computation of the Gaussian mechanism. \yw{Add the reference to the theorem of the Gaussian mechanism.}

To see the second statement, observe that it is a standard univariate Gaussian mechanism. By Weyl's lemma, the smallest singular value satisfies a perturbation bound of $f''(z,\hat{\theta}^p)\|xx^T\|_2 = f''(z,\hat{\theta}^p)\|x\|^2$, since the per-example Hessian is rank-1 in GLM. The stated result again follows from the theorem of the Gaussian mechanism.
\end{proof}

% to go with universal constant proof
  \begin{corollary}[The additional privacy cost]
    If we calibrate $\sigma_2$ such that the Algorithm~\ref{alg:dataset_dependent_report} satisfies the same $(\epsilon,\delta)$-DP as Algorithm~\ref{alg:Alg1}, i.e., when $\epsilon<1$, we could choose $\sigma_2 = \frac{\rho_{\max}}{\epsilon}\sqrt{2\log(1.25/\delta)}$ \footnote{We can alternatively use the optimal calibration via the analytical Gaussian mechanism~\citep{balle2018improving} (or equivalently via GDP) for a tighter calibration that applies to all $\epsilon\geq 0$.}. Then Algorithm~\ref{alg:dataset_dependent_report} satisfies $(\epsilon(z),\delta)$-pDP with
        $$
        \epsilon(z) =\frac{\epsilon^2 (f'')^2\|x\|^4}{8 \rho_{\max}^2 \log(1.25/\delta)} + \frac{\epsilon (f'')\|x\|^2}{\rho_{\max} \sqrt{2}}.$$
    For those cases when $ \frac{(f'')\|x\|^2}{\rho_{\max}}\leq  \frac{|f'|\|x\|}{\beta}$ (which is the case in logistic regression for all $x$ s.t., $\|x\|\leq 1$), the additional overhead in releasing a dataset-dependent pDP is smaller than the ex post pDP bound in Theorem~\ref{thm:pdp_alg1_general}.
    \end{corollary}
    


==> Privately Publishable Per-instance Privacy/subsections/pdp_analysis.tex <==
% !TEX root = ../main.tex

    Our goal in this section is to derive the personalized privacy losses (under Definition~\ref{def:expost_pdp}) associated with observing the output $\hat{\theta}^P$ of objective perturbation. This \emph{ex-post} perspective is highly adaptive and also convenient for our analysis of Algorithm~\ref{alg:Alg1}, whose privacy parameters are a function of the data. Since we are analyzing the per-instance privacy cost of \emph{releasing} $\hat{\theta}^P$, it makes perfect sense to condition the pDP loss on the privatized output of the computation.
     
    %As it turns out, the per-instance privacy losses of releasing $\hat{\theta}^P$ depend on the value of $\hat{\theta}^P$ itself. Below, we introduce a privacy definition convenient for this type of situation.
%
%    \begin{defn} (\textit{Ex-post} per-instance differential privacy)
%        A randomized algorithm $\mathcal{A}$ satisfies $(\epsilon(\cdot), \delta)$-\textit{ex-post} per-instance differential privacy for an individual $z$ and a fixed dataset $D$ if given an outcome $o = \mathcal{A}(D)$, it holds that
%        \begin{align*}
%            &\text{Pr}\big[\mathcal{A}(D) = o \big] \leq e^{\epsilon}\text{Pr}\big[\mathcal{A}(D_{\pm z}) = o\big] + \delta. \\
%            &\text{Pr}\big[\mathcal{A}(D_{\pm z})= o\big] \leq e^{\epsilon}\text{Pr}(\mathcal{A}(D)= o\big] + \delta.
%        \end{align*}
%    \end{defn}
%    

%
%        \begin{defn} (\textit{Ex-post} per-instance differential privacy)
%    	A randomized algorithm $\mathcal{A}$ satisfies $\epsilon(\cdot)$-\textit{ex-post} per-instance differential privacy for an individual $z$ and a fixed dataset $D$ at an outcome $o\in \mathrm{Range}(\cA)$ if 
%    	$$
%    	\left|\log\left(\frac{\text{Pr}\big[\mathcal{A}(D) = o \big]}{\text{Pr}\big[\mathcal{A}(D_{\pm z})= o\big]}\right)\right| \leq \epsilon(o,D,D_{\pm z}). 
%    	$$ 
%    \end{defn}
%    % discuss a bit more...
%    This definition generalizes the ex-post DP definition \citep{ligett2017accuracy} (introduced for a different purpose) to a more adaptive \emph{per-instance} version that depends on a given pair of datasets.
%    %The ex-post DP definition \cite{ligett2017accuracy} was designed to analyze algorithms whose privacy guarantees aren't fixed but rather depend on properties of the computation. 
%    This perspective is convenient for our analysis of Algorithm~\ref{alg:Alg1}, whose privacy parameters are a function of the data. Since we are analyzing the per-instance privacy cost of \emph{releasing} $\hat{\theta}^P$, it makes perfect sense to condition the pDP loss on the privatized output of the computation.
%
%\yw{This is debatable but I've moved the definition to the appendix and this one can be deleted.. some reorganizing  / merging of the text is needed.}

Our first technical result is a precise calculation of the \emph{ex-post} pDP loss of objective perturbation.
    %  \begin{theorem}[Per-instance privacy loss of Algorithm~\ref{alg:Alg1}]
    %     \label{thm:Alg1} 
    %     %\emph{(Per-instance privacy loss of Algorithm~\ref{alg:Alg1})}\newline
    %     Let $J(\theta; D) = L(\theta ; D) + r(\theta) + \frac{\lambda}{2}||\theta||^2$ such that $L(\theta; D) = \sum_i \ell_i(\theta)$, and sample $b \sim \mathcal{N}(0, \sigma^2 I)$. Then for every privacy target $z = (\bm{x}, y)$, releasing $\hat{\theta}^P = \argmin_{\theta \in \Theta} J(\theta; D) + b^T\theta$ satisfies $\epsilon_1(\hat{\theta}^P, D, z)$-\textit{ex-post} per-instance differential privacy with
    %     \begin{align*}
    %         \epsilon(\hat{\theta}^P, D, D_{\pm z}) &\leq 
    %         \log \big(1 + \mu_1(x) \big) + \frac{1}{2\sigma^2}||\nabla \ell_z(\hat{\theta}^P)||^2  +  \frac{1}{\sigma^2}\Big| g^T\nabla \ell_z(\hat{\theta}^P) \Big|,
    %     \end{align*}
    %     where $\mu_1(x) = f''(x^T \hat{\theta}^P)x^T \big(\nabla^2 J(\hat{\theta}^P; D)\big)^{-1}x$, and $g =\nabla J(\hat{\theta}^P ; D)$.
    % \end{theorem}
    
    \begin{theorem}[\emph{ex-post} pDP loss of objective perturbation for a convex loss function]
\label{thm:pdp_alg1_general}

Let $J(\theta; D) = L(\theta ; D) + r(\theta) + \frac{\lambda}{2}||\theta||_2^2$ such that $L(\theta; D)  + r(\theta) = \sum_i \ell(\theta; z_i) + r(\theta)$ is a convex and twice-differentiable regularized loss function, and sample $b \sim \mathcal{N}(0, \sigma^2 I_d)$. Then for every privacy target $z = (x, y)$, releasing $\hat{\theta}^P = \argmin_{\theta \in \mathbb{R}^d} J(\theta; D) + b^T\theta$ satisfies $\epsilon_1(\hat{\theta}^P, D, D_{\pm z})$-\textit{ex-post} per-instance differential privacy with
\begin{align*}
    \epsilon_1(\hat{\theta}^P, D, D_{\pm z} ) =\left| -\log\prod\limits_{j = 1}^d \Big(1 \mp \mu_j \Big) + \frac{1}{2\sigma^2}||\nabla \ell(\hat{\theta}^P; z)||_2^2 \pm \frac{1}{\sigma^2} \nabla J(\hat{\theta}^P;D)^T\nabla \ell(\hat{\theta}^P; z)\right|,
\end{align*}
where $\mu_j = \lambda_j u_j^T\Big(\nabla b(\hat{\theta}^P; D) \mp \sum_{k = 1}^{j - 1} \lambda_k u_k u_k^T \Big)^{-1}u_j $ according to the eigendecomposition $\nabla^2 \ell(\theta; z) = \sum_{k = 1}^{d}\lambda_k u_ku_k^T$.
\end{theorem}
    
    \begin{proof}[Proof sketch]
    	Following the analysis of \citep{chaudhuri2011differentially}, we establish a bijection between the mechanism output $\hat{\theta}^P$ and the noise vector $b$, and use a change-of-variables defined by the Jacobian mapping between $\hat{\theta}^P$ and $b$ in order to rewrite the log-probability ratio in terms of the probability density function of $b$. First-order conditions then allow us to solve directly for the distribution of $b$. To calculate the first term of the above equation, we use the eigendecomposition of the Hessian $\nabla^2 \ell(\hat{\theta}^P; z)$ and recursively apply the matrix determinant lemma. The rest of the proof is straightforward algebra. The full proof is given in Appendix~\ref{app:proofs}.
    \end{proof}
    
    The above expression holds for any convex loss function, but is a bit unwieldy. The calculation becomes much simpler when we assume $\ell(\cdot)$ to be a generalized linear loss function, with inner-product form $\ell(\theta; z) = f(x^T \theta; y)$. For the sake of interpretability, we will defer further discussion of the \emph{ex-post} pDP loss of objective perturbation until after presenting the following corollary.
    
    \begin{corollary}[\emph{ex-post} pDP loss of objective perturbation for GLMs]
    \label{cor:pdp_alg1_linear}
            Let $J(\theta; D) = L(\theta ; D) + r(\theta) + \frac{\lambda}{2}||\theta||_2^2$ such that $L(\theta; D) = \sum_i \ell(\theta; z_i)$ is a linear loss function, and sample $b \sim \mathcal{N}(0, \sigma^2 I_d)$. Then for every privacy target $z = (x, y)$, releasing $\hat{\theta}^P = \argmin_{\theta \in \mathbb{R}^d} J(\theta; D) + b^T\theta$ satisfies $\epsilon_1(\hat{\theta}^P, D, D_{\pm z})$-\textit{ex-post} per-instance differential privacy with
        \begin{align*}
            \epsilon(\hat{\theta}^P, D, D_{\pm z}) &\leq
            \left|-\log \big(1 \pm f''(\cdot)\mu(x) \big) + \frac{1}{2\sigma^2}||\nabla \ell(\hat{\theta}^P; z)||_2^2  \pm  \frac{1}{\sigma^2} \nabla J(\hat{\theta}^P; D)^T\nabla \ell(\hat{\theta}^P; z) \right|,
        \end{align*}
        where $\mu(x) = x^T \big(\nabla^2 J(\hat{\theta}^P; D)\big)^{-1}x$, $\nabla \ell(\hat{\theta}^P; z) = f'(x^T\hat{\theta}^P; y)x$ and $f''(\cdot)$ is shorthand for $f''(\cdot) = f''(x^T \hat{\theta}^P; y)$. The notation $b(\hat{\theta}^P; D)$ means the realization of the noise vector $b$ for which the output of Algorithm \ref{alg:Alg1} will be $\hat{\theta}^P$ when the input dataset is $D$.
    \end{corollary}
 
 
 Note that the quantity $\mu(x)$ in the first term is the \emph{generalized leverage score} \citep{wei1998generalized}, quantifying the influence of a data point on the model fit. The second and third terms are a function of the gradient of the loss function and provide a complementary measure of how well the fitted model predicts individual $z$'s data.
\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/ex_post_logistic.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Visualization of \emph{ex-post} pDP losses for logistic regression ($n = 1000, d = 2$).}
  \label{fig:ex_post}
\end{figure}

Since the \emph{ex-post} pDP is a function of $\hat{\theta}^P$, we don't even need to run Algorithm ~\ref{alg:Alg1} to calculate \emph{ex-post} pDP losses -- we can plug in directly to Corollary ~\ref{cor:pdp_alg1_linear} in order to calculate the pDP distribution induced by any hypothetical $\hat{\theta}^P$. For Figure ~\ref{fig:ex_post}, we use a synthetic dataset $D$ sampled from the unit ball with two linearly separable classes separated by margin $m= 0.4$. Then we solve for $\hat{\theta} = \argmin J(\theta; D)$ with $\lambda = 1$ to minimize the logistic loss, and directly perturb the output by rotating it by angle $\omega \in [0, \frac{\pi}{12}, \frac{\pi}{4}, \frac{\pi}{2}, \frac{3\pi}{4}, \pi]$. We then denote $\hat{\theta}^P := \theta_{+ \omega}$ to mean $\theta$ rotated counter-clockwise by angle $\omega$. The color scale is a function of the \emph{ex-post} pDP loss of data point $z$. 

Figure ~\ref{fig:ex_post} illustrates how the mechanism output $\hat{\theta}^P$ affects the \emph{ex-post} pDP distribution of objective perturbation for our logistic regression problem. For $\omega \in [0, \frac{\pi}{12}]$, the data points closest to the decision boundary have the highest \emph{ex-post} pDP loss. These data points have a strong effect on the learned model and would therefore have high \emph{leverage scores}, making the first term dominate. As the perturbation (and model error) increases, the second and third terms dominate; the more badly a model predicts a data point, the less protection this data point has.

Hidden in this analysis are the $\delta$'s of Theorem ~\ref{thm:alg1}, which along with the choice of $\sigma$ and $\lambda$ could affect which of the three terms is dominant. Fortunately, the probability of outputting something like $\hat{\theta}^P = \theta_{+ \pi}$ is astronomically low for any reasonable privacy setting!


    

    % The quantity $\mu(x)$ is the \emph{generalized leverage score} of the observation $x$. The generalized leverage score is an extension of the leverage score in linear regression to more general estimators and models, as introduced in \citep{wei1998generalized}. In linear regression, it commonly measures the distance between observation $x_i$ and the mean of all $x$ values in the dataset; more generally, it quantifies the influence of observed value $y_i$ on predicted value $\hat{y}_i$ as the instantaneous rate of change of $\hat{y}_i$ with respect to $y_i$.
    
    % The appearance of $\mu(x)$ in the pDP loss of individual $z$ confirms our hunch that $z$ is better protected when their data is ``typical'' (small leverage score) and doesn't exert much influence on the fit of the model to observed data.
    
    % Similarly, the quantity $| \nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)|$ tells us that the per-instance privacy guarantee to $z$ is stronger when the gradients $\nabla J(\hat{\theta}^P; D)$ and $\nabla \ell(\hat{\theta}^P; z)$ are nearly orthogonal. When the value of $| \nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)|$ is small, $\nabla \ell(\hat{\theta}^P; z)$ points roughly in the direction of least change in the objective function at the point $\hat{\theta}^P$.
    
    % The dataset-dependent quantities $\mu_1(x)$ and $| \nabla J(\hat{\theta}^P; D)^T \nabla \ell_z(\hat{\theta}^P)|$ indicate how much influence the data point $z$ exerts on the model's fit. In contrast, the remaining quantity $||\nabla \ell(\hat{\theta}^P; z)||^2$ depends only on $z$ and provides a complementary measure of how well the fitted model predicts individual $z$'s data.

==> Privately Publishable Per-instance Privacy/subsections/privacy_report.tex <==
% !TEX root = ../main.tex

For certain regimes, we may wish to consider privatizing the data-dependent quantities of the \emph{ex-post} pDP losses, at an additional privacy cost, as an alternative to using data-independent bounds. Of course, it only makes sense to do so if we can show that (a) these data-dependent estimates are more accurate than the data-independent bounds; (b) the overhead of releasing additional quantities (the additional privacy cost in terms of both DP and pDP) is not too large; and (c) we can share the pDP losses of the private reporting algorithm using data-independent bounds (so we do not have to recursively publish such reports).

Full details are in the appendix. We show that by adding slightly more regularization than required by \texttt{Obj-Pert} (i.e., making $\lambda$ just a bit larger so that the minimum eigenvalue of the Hessian $H = \nabla^2 J$ is above a certain threshold), we can find a multiplicative bound that estimates $\mu(x) = x^T H^{-1} x$ uniformly for all $x$. We do so by adding noise to the Hessian using a natural variant of "Analyze Gauss" \citep{dwork2014analyze}, hence privately releasing $\overline{\mu^P}:\cX \rightarrow \R$. See Algorithm~\ref{alg:privacy_report} for details.  

For brevity, we use the short-hands $f'(\cdot):= f'(x^T \hat{\theta}^P; y)$ and $f''(\cdot) := f''(x^T\hat{\theta}^P; y)$, where $\ell(\theta; z) = f(x^T\theta; y)$ for GLMs. $F^{-1}_{\mathcal{N}(0, 1)}$ is the inverse CDF of the standard normal distribution, and $F^{-1}_{GOE(d)}$ is the inverse CDF of the largest eigenvalue of the Gausian Orthogonal Ensemble (GOE) matrix, whose distribution is calculated exactly by \citep{chiani2014distribution}. Algorithm ~\ref{alg:privacy_report} specializes to GLMs for clarity of presentation, but we could adapt it to any convex loss function by replacing the GLM-specific bounds with the more general ones.

We implicitly assume that the data analyst has already decided the privacy budgets $\epsilon_2$ and $\epsilon_3$ for the data-dependent release of the gradient (third term of $\epsilon_1(\cdot)$) and of the Hessian (first term of $\epsilon_1(\cdot)$). Inputs $\sigma_2$ and $\sigma_3$ are then calibrated to achieve $(\epsilon_2, \rho)$-DP and $(\epsilon_3, \rho)$-DP, respectively.

%We now have calculated the \emph{ex-post} pDP losses of the objective perturbation algorithm, and have the tools to privately release these pDP losses. Algorithm ~\ref{alg:privacy_report} utilizes the data-independent and data-dependent bounds described in Section ~\ref{release_pdp} in order to release private estimates of the pDP losses of objective perturbation for generalized linear models. Algorithm ~\ref{alg:privacy_report} uses the high-probability, data-independent bound stated in Theorem~\ref{thm:data_indep_third} to release the third term of the pDP loss, and user input determines whether to compute $\overline{\mu^P}$, the private estimate of $\mu(x)$, with the data-independent bound discussed in Theorem~\ref{thm:data_indep_first} or with the data-dependent method described in Section ~\ref{sub:data_dep_bounds}.

        \begin{algorithm}[H]
        \caption{Privacy report for \texttt{Obj-Pert} on GLMs}
        \label{alg:privacy_report}
        \begin{algorithmic}
            \STATE {\bfseries Input:} $\hat{\theta}^p \in \mathbb{R}^d$ from \texttt{Obj-Pert}, noise parameter $\sigma,\sigma_2, \sigma_3$; regularization parameter $\lambda$; Hessian $H := \sum_i\nabla^2\ell(\hat{\theta}^p; z_i) + \lambda I_d$, Boolean B $\in$ [\texttt{DATA-INDEP}, \texttt{DATA-DEP}], failure probability $\rho$
            \STATE {\bfseries Require: $\lambda \geq 2 \sigma_3 F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$}
            \STATE {\bfseries Output:} Reporting function $\tilde{\epsilon}: (x,y),\delta \rightarrow \R_+^3$
            \IF {B = \texttt{DATA-INDEP}}
            \STATE Set $\epsilon_2(\cdot):= 0, \epsilon_3(\cdot) := 0$.
            \vspace{2pt}
            \STATE Set $\overline{g^P}(z) := \sigma ||f'(\cdot)x||_2 F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2})$ and set $\overline{\mu^p}(x) := \frac{\|x\|^2}{\lambda}$. 
            % \STATE Set $\underline{g^P}(z) := -\overline{g^P}(z)$.
            % \vspace{2pt}
            % \STATE Set 
            % % Set $\underline{\mu^p}(x) := 0.$
            %\vspace{4pt}
            \ELSIF {B = \texttt{DATA-DEP}}
            \STATE Privately release $\hat{g}^p$ by Algorithm ~\ref{alg:Alg_gp} with parameter $\sigma_2$.
            \STATE Set $\epsilon_2(\cdot)$ according to Theorem $\ref{thm:gp_pdp}$.
             \STATE Set {\small $\overline{g^P}(z) := \min\left\{f'(\cdot) [\hat{g}^P(z)]^Tx + \sigma_2 ||f'(\cdot)x||_2 F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2}),\; \sigma ||f'(\cdot)x||_2 F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2})\right\}.$}
            %  \STATE Set $\underline{g^P}(z) := f'(\cdot) [\hat{g}^P]^Tx - \sigma_2 ||f'(\cdot)x||_2F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2}).$
            \STATE Privately release $\hat{H}^p$ by a variant of "Analyze Gauss"\footnotemark with parameter $\sigma_3$.
            \STATE Set $\epsilon_3(\cdot)$  according to Statement 2 of Theorem~\ref{thm:master_thm_reporting}.
            \STATE Set $\overline{\mu^p}(x) = \frac{3}{2}x^T [\hat{H}^p]^{-1} x$.
            % Set $\underline{\mu^p}(x) := \frac{1}{2}x^T [\hat{H}^p]^{-1} x$.
            \vspace{2pt}
            \ENDIF
            % \STATE Let $\omega \in [-1, 1], g^P \in \Big[\overline{g^P}(z), \underline{g^P}(z)\Big], \mu^P \in \Big[\overline{\mu^P}(x), \underline{\mu^P}(x)\Big]$.
            \vspace{2pt}
            \STATE Set $\overline{\epsilon_1^p}(z):= \big| -\log \big(1 -  f''(\cdot)\overline{\mu^p}(x) \big)  \big| + \frac{||f'(\cdot)x||_2^2}{2\sigma^2} +  \frac{\big|\overline{g^P}(z)\big|}{\sigma^2}.$
            %  \STATE Set $\overline{\epsilon_1^p}(z):= \max\limits_{\omega, g^P,\: \mu^P}\left\{
            % \left|-\log \big(1 + \omega f''(\cdot)\mu^p \big) + \frac{||f'(\cdot)x||^2}{2\sigma^2}  + \omega  \frac{g^P}{\sigma^2} \right|\right\}$.
            \STATE Output the function $\tilde{\epsilon}(z) := \big(\overline{\epsilon_1^p}(z), \epsilon_2(z), \epsilon_3(z)\big)$.
            \end{algorithmic}
        \end{algorithm}
        \footnotetext{Instead of adding ``analyze-gauss'' noise, we sample from the Gaussian Orthogonal Ensemble (GOE) distribution to obtain a random matrix (Appendix~\ref{app:analyze_gauss}). Under this model we show that $\tau$ is on the order of $O(\sqrt{d}(1 + \log(C/\rho)^{3/2}))$.}
    
        %  \begin{algorithm}[H]
        % \caption{Privacy report for \texttt{Obj-Pert} on GLMs}
        % \label{alg:privacy_report}
        % \begin{algorithmic}
        %     \STATE {\bfseries Input:} $\hat{\theta}^p$ from \texttt{Obj-Pert}, noise parameter $\sigma,\sigma_2$; regularization parameter $\lambda$; Hessian $H := \sum_i\nabla^2\ell(\hat{\theta}^p; z_i) + \lambda I_d$, Boolean B $\in$ [\texttt{DATA-INDEP}, \texttt{DATA-DEP}], failure probability $\rho$
        %     \STATE {\bfseries Output:} Reporting function $\tilde{\epsilon}: (x,y),\delta \rightarrow \R_+^2$
        %     \IF {B = \texttt{DATA-INDEP}}
        %     \STATE Set $\epsilon_2(\cdot) := 0$. 
        %     \STATE Set $\overline{\mu^p}(x) := \frac{\|x\|^2}{\lambda}$.
        %     \ELSIF {B = \texttt{DATA-DEP}}
        %      \STATE Privately release $\hat{H}^p$ by a variant of "Analyze Gauss"\footnotemark with parameter $\sigma_2$. 
        %     % \STATE Privately release $\hat{H}^p$ by Algorithm~\ref{alg:release_H} with parameter $\sigma_2$. 
        %      \STATE Set $\epsilon_2(\cdot)$  according to Statement 2 of Theorem~\ref{thm:master_thm_reporting}.
        %     \STATE Set $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$.
        %     \STATE \IF{$\lambda \geq  2 \tau \sigma_2$}
        %     \STATE Set $\overline{\mu^p}(x) = \frac{3}{2}x^T [\hat{H}^p]^{-1} x$.
        %     \ENDIF            \ENDIF
        %      \STATE Set $\overline{\epsilon_1^p}(z):= \max\left\{
        %     \left|-\log \big(1 \pm f''(\cdot)\overline{\mu^p}(x) \big) + \frac{|f'(\cdot)|^2||x||^2}{2\sigma^2}  \pm  \frac{|f'(\cdot)|||x|| F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2})}{\sigma} \right|\right\}$.
        %     \STATE Output the function $\tilde{\epsilon}(z) := (\overline{\epsilon_1^p(z)}, \epsilon_2(z))$.
        %     \end{algorithmic}
        % \end{algorithm}
        % \footnotetext{Instead of adding ``analyze-gauss'' noise, we sample from the Gaussian Orthogonal Ensemble (GOE) distribution to obtain a random matrix (Appendix A). Under this model we show that $\tau$ is on the order of $O(\sqrt{d}(1 + \log(C/\rho)^{3/2}))$.}

    

    Note that the pDP functions $\epsilon_2(\cdot)$ and $\epsilon_3(\cdot)$ -- which we use to report the additional pDP losses of releasing the private estimates of the gradient and the Hessian -- do not depend on the dataset, and thus are not required to be separately released. The privately released pDP functions depend on $\hat{\theta}^P$; to reduce clutter, we omit this parameter in our presentation of Algorithm ~\ref{alg:privacy_report}.
   
    
    %     \begin{theorem}\label{thm:master_thm_reporting}
    % There is a universal constant $C$ such that if $\lambda > C\sigma_2\sqrt{d}(1+(\log(1/\rho))^{2/3})$, then Algorithm~\ref{alg:privacy_report} satisfies the following properties
    % \begin{enumerate}
    %     %\item  $\frac{\rho_{\max}}{\sqrt{2}\sigma_2}$- (worst-case) Gaussian DP.
    %     %\item  $\frac{f''(x,\hat{\theta}^p) \|x\|^2}{\sqrt{2}\sigma_2}$-per-instance Gaussian DP.
    %     \item $(\frac{\beta^2}{4\sigma_2^2} + \frac{\beta\sqrt{\log(1/\delta)}}{\sigma_2},\delta)$-DP
    %     \item $(\frac{f''(x,\hat{\theta}^p)^2 \|x\|^4}{4\sigma_2^2} + \frac{f''(x,\hat{\theta}^p)\|x\|^2\sqrt{\log(1/\delta)}}{\sigma_2},\delta)$-pDP for all $x\in\cX$ and $0 \leq \delta<1$.
    %     % \item (Utility of releasing $\mu(x)$): with probability $1-\rho$, simultaneously for all $x\in\cX$
    %     % $$
    %     % \mu(x)\leq \overbar{}
    %     % $$
        
    %     \item   For a fixed input $z$, and all $\rho>0$, the privately released privacy report $\tilde{\epsilon}(\cdot)$ satisfies that $\epsilon_1(z,\hat{\theta}^p) \leq \overline{\epsilon^p}_1(z,\hat{\theta}^p) \leq \max\{12,\sqrt{2 \log(2/\rho)}\}\epsilon_1(z,\hat{\theta}^p)$ with probability $1-2\rho$ where $\epsilon_1$ is the expression from Theorem~\ref{thm:pdp_alg1_general}.
    %     % \item With probability $1-\rho$,  \emph{simultanesouly} for all $n$ users in the dataset, $\epsilon_1(z,\hat{\theta}^p) \leq \overline{\epsilon^p}_1(z,\hat{\theta}^p) \leq 2 \sqrt{\log n} \epsilon_1(z,\hat{\theta}^p)$
    %     % \item With probability $1-\rho$, \emph{uniformly} For all $(x,y)\in\R^d\times \mathcal{Y},$ the \emph{ex post} pDP loss 
    %     % $\epsilon(z,\hat{\theta}^p) \leq $
        
        
    % \end{enumerate}
    % \end{theorem}
    
            \begin{theorem}\label{thm:master_thm_reporting}
    There is a universal constant $C$ such that if $\lambda > C\sigma_2\sqrt{d}(1+(\log(1/\rho))^{2/3})$, then Algorithm~\ref{alg:privacy_report} satisfies the following properties
    \begin{enumerate}
        \item $(\frac{\xi^2}{2\sigma_2^2}+\frac{\beta^2}{4\sigma_3^2} + \sqrt{\frac{\xi^2}{\sigma_2^2}+\frac{\beta^2}{2\sigma_3^3}}\sqrt{2\log(1/\delta)},\delta)$-DP
        \item $ ( \frac{f'(\hat{\theta}^p; z)^2\|x\|^2}{2\sigma_2^2} + \frac{f''(\hat{\theta}^p; z)^2 \|x\|^4}{4\sigma_3^2} + \sqrt{\frac{f'(\hat{\theta}^p; z)^2\|x\|^2}{\sigma_2^2} + \frac{f''(\hat{\theta}^p; z)^2\|x\|^4}{2\sigma_3^2}} \sqrt{2\log(1/\delta)},\delta)$-pDP for all $x\in\cX$ and $0 \leq \delta<1$.

        \item   For a fixed input $z$ and $D$, and all $\rho>0$, the privately released privacy report $\tilde{\epsilon}(\cdot)$ satisfies that  
        $\epsilon_1(\hat{\theta}^p, D, D_{\pm z}) \leq \overline{\epsilon^p_1}(z)
        \leq 12\epsilon_1(\hat{\theta}^p, D, D_{\pm z}) + \frac{|f'(\cdot)|\|x\|}{\sigma_2}\sqrt{2 \log(2/\rho)}$ with probability $1-3\rho$ where $\epsilon_1(\cdot)$ is the expression from Theorem~\ref{thm:pdp_alg1_general}.
    \end{enumerate}
    \end{theorem}
    
    % \begin{proof}
    % Under the stated condition, by Lemma~\ref{lem:lambda_GOE}, we know that $\lambda$ is sufficiently large in the first ``if'' condition and we will be using the non-adaptive approach via  
    % $\overline{\mu^p}(x) = \frac{3}{2}x^T [\hat{H}^p]^{-1} x$ without separately releasing $\hat{\lambda}_{\min}$.
    
    % The privacy guarantees (Statement 1-3) follow directly from the pDP analysis in Theorem~\ref{thm:pdp_of_H_lambda_min} that analyzes the release of $H$ by adding a GOE noise matrix.
    
    % By the result follows from Proposition~\ref{prop:utility_H_large_lambda} we know that with probability $1-\rho$, for all $x$ 
    % $$\mu(x) \leq \frac{3}{2}\hat{\mu}^p(x)\leq 3\mu(x)$$
    
    % For all $a\geq -1$
    % $
    % \frac{a}{1+a} \leq \log(1+a) \leq a.
    % $
    % By our condition that $\|x\|_2\leq 1$ and $\lambda > 2$ and $\rho_{\max}\leq 1$, as well as the pointwise minimum in the construction of $\overline{\mu^p}$, we have that
    % $\frac{f''\overline{\mu^p}}{2}\leq \max\{\log(1+f''\overline{\mu^p}), -\log(1-f''\overline{\mu^p}\} \leq 2 f''\overline{\mu^p}$.
    % Thus 
    % $$
    % \log(1+\mu) \leq \mu \leq \overline{\mu^p}\leq 2\log(1+\overline{\mu^p}) \leq 2 \overline{\mu^p} \leq 3 \hat{\mu}^p\leq 6\mu \leq 12\log(1+\mu),
    % $$
    % and similarly
    % $$
    % -\log(1-\mu) \leq 2\mu \leq 2\overline{\mu^p}\leq -2\log(1-\overline{\mu^p}) \leq 4\overline{\mu^p} \leq 6 \hat{\mu}^p \leq  12 \mu \leq -12\log(1-\mu).
    % $$
    % This concludes the factor $12$ multiplicative approximation.
    % \end{proof}
    \noindent\textbf{Accurate approximation with low privacy cost.} 
    This theorem shows that if we %choose $\sigma_2\asymp \sigma_3 \asymp \sigma$ and 
    use a slightly larger $\lambda$ in ObjPert then we get an upper bound of the pDP for each individual $z$ up to a multiplicative and an additive factor.  The multiplicative factor is coming from a multiplicative approximation of $-\log \big(1 \pm f''(\cdot)\mu(x) \big)$ and the additive error is due to the additional noise added for releasing the third term $\frac{1}{\sigma^2} \nabla J(\hat{\theta}^P; D)^T\nabla \ell(\hat{\theta}^P; z)$.
    %\emph{constant multiplicative approximation} if the $-\log \big(1 \pm f''(\cdot)\mu(x) \big)$ term dominates $\epsilon_1(z)$; and an additive approximation if the $\frac{1}{\sigma^2} \nabla J(\hat{\theta}^P; D)^T\nabla \ell(\hat{\theta}^P; z)$ term dominates. In the latter regime, the data-independent bound will give a comparable additive error with $\sigma_2$ replaced by $\sigma$.
    The additional DP and pDP losses for releasing $H$ and $g$ are comparable to the DP and pDP losses in Objective Perturbation itself if $\sigma_2\asymp \sigma_3 \asymp \sigma$.
     
    Moreover, while using a large $\lambda$ may appear to introduce additional bias, the required choice of $\lambda \asymp \sqrt{d}\sigma$ is actually exactly the choice to obtain the minimax rate in general convex private ERM \citep{bassily2014private} (Figure~\ref{fig:lambda_utility} demonstrates the impact of increasing $\lambda$). 
    % We discuss a more adaptive algorithm in the appendix that adapts to a well-conditioned $H$ matrix that avoids using a large $\lambda$ and achieves a stronger approximation of the leverage score $\mu(\cdot)$, which will result in a significantly better approximation of $\epsilon_1$ if the $-\log(1-\mu(\cdot))$ term is the dominating term in $\epsilon_1$ (as is the case when $\lambda$ is small).
    
    %A global multiplicative approximation is not achievable because the pDP for some lucky individual may happen to be arbitrarily close to $0$.
    
    \noindent\textbf{Joint DP interpretation.} Finally, we can also interpret our results from a joint-DP perspective \citep{kearns2014mechanism}.  Given any realized output $\hat{\theta}^p\in \R^d$, the tuple of $\{\tilde{\epsilon}(z_1,\hat{\theta}^p),...,\tilde{\epsilon}(z_1,\hat{\theta}^p)\}$ satisfies joint DP with the same $\epsilon$ parameter as in Theorem~\ref{thm:master_thm_reporting}. This follows from the billboard lemma \citep{hsu2016private}.
    
%    We include more details in the Appendix. 
    
    % \begin{corollary}[The additional privacy cost]
    % If we calibrate $\sigma_2$ such that the Algorithm~\ref{alg:dataset_dependent_report} satisfies the same $(\epsilon,\delta)$-DP as Algorithm~\ref{alg:Alg1}, i.e., when $\epsilon<1$, we could choose $\sigma_2 = \frac{\rho_{\max}}{\epsilon}\sqrt{2\log(1.25/\delta)}$ \footnote{We can alternatively use the optimal calibration via the analytical Gaussian mechanism~\citep{balle2018improving} (or equivalently via GDP) for a tighter calibration that applies to all $\epsilon\geq 0$.}. Then Algorithm~\ref{alg:dataset_dependent_report} satisfies $(\epsilon(z),\delta)$-pDP with
    %     $$
    %     \epsilon(z) =\frac{\epsilon^2 (f'')^2\|x\|^4}{8 \rho_{\max}^2 \log(1.25/\delta)} + \frac{\epsilon (f'')\|x\|^2}{\rho_{\max} \sqrt{2}}.$$
    % For those cases when $ \frac{(f'')\|x\|^2}{\rho_{\max}}\leq  \frac{|f'|\|x\|}{\beta}$ (which is the case in logistic regression for all $x$ s.t., $\|x\|\leq 1$), the additional overhead in releasing a dataset-dependent pDP is smaller than the ex post pDP bound in Theorem~\ref{thm:pdp_alg1_general}.
    % \end{corollary}
    % \begin{proof}
    % $$\frac{\epsilon^2 (f'')^2\|x\|^4}{8 \rho_{\max}^2 \log(1.25/\delta)} + \frac{\epsilon (f'')\|x\|^2 \sqrt{\log(1/\delta)}}{\rho_{\max} \sqrt{2\log(1.25/\delta)}}.$$
    % \end{proof}
    % \begin{corollary}[Joint DP interpreation.]
    % Given any realized output $\tilde{\theta}^p\in \R^d$. The tuple of $\{\tilde{\epsilon}(z_1,\hat{\theta}^p),...,\tilde{\epsilon}(z_1,\hat{\theta}^p)\}$ satisfies joint-DP and joint-pDP with the same $\epsilon$ parameter as in the Theorem~\ref{thm:master_thm_reporting}. \yw{@Rachel, could you check whether we should add \emph{ex post} here?} 
    % \end{corollary}
    % \begin{proof}
    % Apply the standard and per-instance version of the billboard lemmas.
    % \end{proof}
    
    %     The results stated above provide a utility guarantee for each fixed input, however we could also make it a stronger uniform convergence result.
        
      
    % \begin{proof}
    % $$\frac{\epsilon^2 (f'')^2\|x\|^4}{8 \rho_{\max}^2 \log(1.25/\delta)} + \frac{\epsilon (f'')\|x\|^2 \sqrt{\log(1/\delta)}}{\rho_{\max} \sqrt{2\log(1.25/\delta)}}.$$
    % \end{proof}
    % \begin{corollary}[Joint DP interpreation.]
    % Given any realized output $\tilde{\theta}^p\in \R^d$. The tuple of $\{\tilde{\epsilon}(z_1,\hat{\theta}^p),...,\tilde{\epsilon}(z_1,\hat{\theta}^p)\}$ satisfies joint-DP and joint-pDP with the same $\epsilon$ parameter as in the Theorem~\ref{thm:master_thm_reporting}.  
    % \end{corollary}


==> Privately Publishable Per-instance Privacy/subsections/problem_setting.tex <==
% !TEX root = ../main.tex

We consider a general family of problems known as \emph{private empirical risk minimization} (ERM), which aim to approximate the solution to an ERM problem while preserving privacy. That is, we wish to privately solve optimization problems of the form
    \begin{align*}
        \hat{\theta} &= \argmin_{\theta \in \Theta}L(\theta ; D) + r(\theta),
    \end{align*}
    where $r(\theta)$ is a regularizer and $L(\theta ; D)= \sum_{i = 1}^n \ell(\theta; z_i)$ a loss function. Throughout, we assume that $\ell(\theta; z)$ and $r(\theta)$ are convex and  twice-differentiable with respect to $\theta$. Dataset $D$ is given by $D = \{ z_i\}_{i = 1}^n$, and $z_i = (x_i, y_i)$ for $x_i \in \mathcal{X} \subseteq \mathbb{R}^d$ and $y \in \mathcal{Y} \subseteq \mathbb{R}$, where $||x||_2 \leq 1$ and $|y| \leq 1$. We consider only unconstrained optimization over $\Theta = \mathbb{R}^d$.
    

    % The loss function has a special structure in that $\ell(\cdot)$ takes the inner-product form $\ell(\theta; z_i) = f(x^T \theta; y_i)$. To make this expression less cumbersome, we will sometimes abbreviate $f(x_i^T \theta; y_i):= \ell_i(\theta)$ to indicate the linear loss function with respect to data point $z_i = (x_i, y_i)$. Furthermore, we assume $||\nabla \ell(\theta; z_i)||_2 \leq \beta$ for all $z_i \in \mathcal{X} \times \mathcal{Y}$ and $\theta \in \Theta$.
    
    % Our pDP analysis will consider objective perturbation, a well-regarded approach for differentially private ERM. We review this algorithm and its privacy guarantees in the next section.

% To make this expression less cumbersome, we will sometimes abbreviate $f(x_i^T \theta; y_i):= \ell_i(\theta)$ to indicate the linear loss function with respect to data point $z_i = (x_i, y_i)$. 

% empirical risk minimization definition, J(\theta)
% x drawn from unit ball, ||x|| <= 1
% linear loss function...generalized linear models l(\theta; z_i) - l(x_i^T \theta; y_i)
% assume bounded first- and second- order derivatives (common assumption)
% adjacent datasets D (fixed), D_{\pm z} is the dataset obtained by either adding or removing z to D
% leave one out aDP
% adversaries...talk about later?


==> Privately Publishable Per-instance Privacy/subsections/related_work.tex <==
% !TEX root = ../main.tex

This paper builds upon \citep{wang2019per}, which proposed the per-instance DP framework and left as an open question the matter of publishing the pDP losses. We extend the pDP framework to an \emph{ex-post} setting to provide privacy guarantees that adapt even more fluidly to data-dependent properties of our algorithms. Another fundamental ingredient in our privacy analysis is the objective perturbation algorithm (\texttt{Obj-Pert}) of \citep{chaudhuri2011differentially}, further analyzed by \citep{kifer2012private}, which privately releases the minimizer of an empirical risk by adding a linear perturbation to the objective function before optimizing. 

Per-instance DP and \emph{ex-post} per-instance DP belong to a growing family of DP definitions that provide a more fine-grained characterization of the privacy loss. Among these are data-dependent DP \citep{papernot2018}, which conditions on a fixed dataset; personalized DP \citep{ghosh2011selling, ebadi2015differential, liu2015fast}, which conditions on a fixed individual’s datapoint; and \emph{ex-post} DP \citep{ligett2017accuracy}, which conditions on the realized output of the algorithm. Per-instance DP conditions on both a fixed dataset and a fixed individual’s datapoint, and \emph{ex-post} per-instance DP adapts even further to the realized output of the algorithm. A more detailed comparison of these DP variants is included in the supplementary materials.

Other data-adaptive methodologies include propose-test-release \citep{dwork2009differential} and local sensitivity \citep{nissim2007smooth}. In addition, Bayesian differential privacy \citep{triastcyn2020bayesian} provides data-dependent privacy guarantees that afford strong protection to "typical" data by making distributional assumptions about the sensitive data. The R\'enyi-DP-based privacy filters of \citep{feldman2020individual} are also closely related to our work; the authors study composition of personalized (but not per-instance) privacy losses using adaptively-chosen privacy parameters.

==> Privately Publishable Per-instance Privacy/subsections/release_pdp.tex <==
% !TEX root = ../main.tex

    Next we consider: after having released $\hat{\theta}^P$ and calculated the per-instance privacy losses of doing so, how do we privately release these pDP losses? Our goal is to allow any individual $z\in \cZ$ (in the dataset or not) to know her privacy loss while preserving the privacy of others in the dataset.
    %We will first introduce the joint per-instance DP framework to help us with this task.
    
    % There are several challenges. The first and foremost is that how to even define the problem.  For example, what is the output space of such a private release? We cannot just output the tuple of the pDP losses for $z\in D$ because it is equally valid for $z\notin D$, and if we restrict it to a vector of $n$, then the dimensionality of the output itself can be used to distinguish $D$ and $D'$.  Also, who are the attackers and what do they observe?  $\epsilon_1(\hat{\theta}^P, D, z)$ is fundamentally a quantity specific to an individual $z$,  and ideally we want to show the private release only to $z$. In this sense, $z$ would be an attacker on other data points, in this sense for each $z\in \cZ$ there is a separate DP release problem.
    %  Secondly, users could collude to gain more information. There are many individuals in the dataset or even more outside the dataset and we cannot privately release the pDP loss for each separately and then appeal to composition. %There are simply too many. 
    %  Thirdly, a DP algorithm to release the pDP losses will incur additional privacy losses and may require a next level of DP algorithm to release these new pDP losses \emph{recursively}.   If the overhead  for releasing pDP losses are much larger than the pDP losses themselves, then it defeats the purpose.
     
    % Our idea is to solve these challenges is to privately release the \emph{sufficient statistics} of the data $D$ that needs to be used for computing $\epsilon_1(\hat{\theta}^P, D, z)$, so the output is a function of only $z$. This allows any individual could plug in their own data to obtain an estimate of their pDP loss (See Figure~\ref{fig:illus} for an illustration.)  
    
%    is to release the \emph{sufficient statistics} of the data $D$ that needs to be used for computing this function, so that any individual could plug in their own data to obtain an estimate of their pDP loss (See Figure~\ref{fig:illus} for an illustration.) 
    
   Observe that the expression from Theorem~\ref{thm:pdp_alg1_general} depends on the dataset $D$ only through two quantities: the leverage score $\mu(x) = x^T \big(\nabla^2 J(\hat{\theta}^P; D)\big)^{-1}x$ and the inner product $\nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)$. As a result, if we can find a data-independent bound for these two terms, or privately release them with only a small additional privacy cost, then we are done.
   
   \subsubsection{Data-independent bound of \emph{ex-post} pDP losses}% for a convex loss function}
   \label{sub:data_indep_bounds}
   
   Below, we present a pair of lemmas which will allow us to find a high-probability, data-independent bound on the \emph{ex-post} pDP loss.
   
   \begin{theorem}
   \label{thm:data_indep_first}
   Suppose $\ell(\cdot)$ is a function with continuous second-order partial derivatives. Then
%   Let $\ell(\cdot)$ be $\beta$-smooth, such that $\nabla^2 \ell(\theta; z) \prec \beta I_d$ for all $\theta \in \mathbb{R}^d$ and $z \in \mathcal{Z}$. 
   \begin{align*}
       \left| -\log\prod\limits_{j = 1}^d \Big(1 \mp \mu_j \Big) \right| \leq -\sum_{j=1}^d\log(1 - \frac{\lambda_j}{\lambda}),
   \end{align*}
   where $\mu_j = \lambda_j u_j^T\Big(\nabla \mathbf{b}(\hat{\theta}^P; D) \mp \sum_{k = 1}^{j - 1} \lambda_k u_k u_k^T \Big)^{-1}u_j$ according to the eigendecomposition $\nabla^2 \ell(\hat{\theta}^P; z) = \sum_{k = 1}^{d}\lambda_k u_ku_k^T$. When specializing to linear loss functions such that $\ell(\theta; z) = f(x^T \theta; y)$, $\lambda_j=0$ for all $j>1$ and the above bound can be simplified to $-\log\left(1 - f''(x^T\hat{\theta}^P; y)||x||_2^2/\lambda\right)$.
   \end{theorem}
   
   \begin{theorem}\label{thm:data_indep_third}
   Let $\hat{\theta}^P$ be a random variable such that $\hat{\theta}^P = \argmin \left(J(\theta; D) + b^T \theta \right)$ as in (\ref{op}), where $b \sim \mathcal{N}(0, \sigma^2I_d)$ and $\ell(\theta; z)$ is a convex and twice-differentiable loss function. Then for $z \in \mathcal{Z}$, the following holds with probability $1 - \rho$:
   \begin{align*}
       \left|\nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)\right| \leq \sigma \sqrt{2 \log(2d/\rho)}\|\nabla \ell(\hat{\theta}^P; z)\|_1.
   \end{align*}
     For linear loss functions the bound can be substantially strengthened to
     \begin{align*}
         \left|\nabla J(\hat{\theta}^P; D)^T\nabla \ell(\hat{\theta}^P; z) \right| \leq f'(x^T\hat{\theta}^p;y)\sigma ||x||_2 \sqrt{2 \log (2/\rho)}.
     \end{align*}
   \end{theorem}
%For an arbitrary convex loss function, the data-independent bound on \emph{ex-post} pDP loss depends on dimension $d$. Fortunately, we can remove this dimension-dependence when we consider bounding the \emph{ex-post} pDP loss for linear loss functions.
% to a completely dimension-free bound.
    %     \begin{theorem}
    %  \label{thm:data_indep_third_glm}
    %  Let $\ell(\cdot)$ be a linear loss function such that $\ell(\theta; z) = f(x^T \theta; y)$, and let $\hat{\theta}^P = \argmin \left(J(\theta; D) + b^T \theta \right)$ as in (\ref{op}). Then with probability $1 - \delta$,
    %  \begin{align*}
    %      \left|\nabla J(\hat{\theta}^P; D)^T\nabla \ell(\hat{\theta}^P; z) \right| \leq \sigma || \nabla \ell(\hat{\theta}^P; z) || \sqrt{2 \log (2/\delta)}.
    %  \end{align*}
    %  \end{theorem}
We make a few observations on the bounds. First, the general bound in Theorem~\ref{thm:data_indep_third} holds simultaneously for all $z$ and it depends only logarithmically in dimension when the features are \emph{sparse}. Second, the bound for a linear loss function is dimension-free and somewhat surprising because we are actually bounding an inner product of two \emph{dependent} random vectors (both depend on $\hat{\theta}^P$).
    
Finally, we remark that the bounds in this section are data-independent in that they do not depend on the rest of the dataset beyond already released information $\hat{\theta}^P$. It allows us to reveal a pDP bound of each individual when she plugs in her own data without costing any additional privacy budget! 
%The bounds themselves are  are also adaptive in that they depend on the data points themselves.
   
   
 %    \subsubsection{Data-independent bound of \emph{ex-post} pDP loss for a linear loss function}
     

     
    %  \begin{lemma}
    % \label{thm:data_indep_first_glm}
    %  Let $\ell(\cdot)$ be a linear loss function such that $\ell(\theta; z) = f(x^T \theta; y)$, and choose $\lambda$ such that $\frac{f''(x^T\theta)||x||^2}{\lambda} \leq 1$ for all $\theta \in \mathbb{R}^d$ and $z \in \mathcal{Z}$. Let $\hat{\theta}^P = \argmin \left(J(\theta; D) + b^T \theta \right)$ as in (\ref{op}). Then for any $z = (x, y) \in 
    %  \mathcal{Z}$ ,
    %  \begin{align*}
    %      \big| -\log\big(1 \pm f''(x^T\hat{\theta}^P)\mu(x)\big)\big| \leq -\log\left(1 - \frac{f''(x^T\hat{\theta}^P)||x||^2}{\lambda}\right).
    %  \end{align*}
    %  \end{lemma}
    %  The above lemma follows from the upper bound $\mu_1(x) = x^T H^{-1}  x\leq \frac{||x||^2}{\lambda}$, where $H = \nabla^2 J(\hat{\theta}^P; z)$ is the Hessian of the objective function.
     

%\subsubsection{Data-dependent bound of \emph{ex-post} pDP loss}
%   \label{sub:data_dep_bounds}


  
    % \begin{proof}
    % Under the stated condition, by Lemma~\ref{lem:lambda_GOE}, we know that $\lambda$ is sufficiently large in the first ``if'' condition and we will be using the non-adaptive approach via  
    % $\overline{\mu^p}(x) = \frac{3}{2}x^T [\hat{H}^p]^{-1} x$ without separately releasing $\hat{\lambda}_{\min}$.
    
    % The privacy guarantees (Statement 1-3) follow directly from the pDP analysis in Theorem~\ref{thm:pdp_of_H_lambda_min} that analyzes the release of $H$ by adding a GOE noise matrix.
    
    % By the result follows from Proposition~\ref{prop:utility_H_large_lambda} we know that with probability $1-\rho$, for all $x$ 
    % $$\mu(x) \leq \frac{3}{2}\hat{\mu}^p(x)\leq 3\mu(x)$$
    
    % For all $a\geq -1$
    % $
    % \frac{a}{1+a} \leq \log(1+a) \leq a.
    % $
    % By our condition that $\|x\|_2\leq 1$ and $\lambda > 2$ and $\rho_{\max}\leq 1$, as well as the pointwise minimum in the construction of $\overline{\mu^p}$, we have that
    % $\frac{f''\overline{\mu^p}}{2}\leq \max\{\log(1+f''\overline{\mu^p}), -\log(1-f''\overline{\mu^p}\} \leq 2 f''\overline{\mu^p}$.
    % Thus 
    % $$
    % \log(1+\mu) \leq \mu \leq \overline{\mu^p}\leq 2\log(1+\overline{\mu^p}) \leq 2 \overline{\mu^p} \leq 3 \hat{\mu}^p\leq 6\mu \leq 12\log(1+\mu),
    % $$
    % and similarly
    % $$
    % -\log(1-\mu) \leq 2\mu \leq 2\overline{\mu^p}\leq -2\log(1-\overline{\mu^p}) \leq 4\overline{\mu^p} \leq 6 \hat{\mu}^p \leq  12 \mu \leq -12\log(1-\mu).
    % $$
    % This concludes the factor $12$ multiplicative approximation.
    % \end{proof}




  
















%   As a result, if we can find a data-independent bound for these two terms, or privately release $ \nabla J(\hat{\theta}^P; D)$ and $H^{-1}$ with small overheads, then we are done.  This is exactly what we propose to do with the Gaussian mechanism in Algorithm~\ref{alg:Alg2}~and~\ref{alg:Alg3}.  
   
%   The following theorems analyzes the pDP and ex post pDP of these two algorithms.
   
%       \begin{theorem} 
%   	\label{thm:alg2_pdp}
%   	Let $\hat{\theta}^P$ be fixed, Algorithm~\ref{alg:Alg2} satisfies
%   	\vspace{-1em}
%   	\begin{enumerate}
%   		\itemsep0em
%   		   		\item $\epsilon_2(o,D,D_{\pm z})$-ex post pDP with probability $1-\delta$,
%   		\item $(\epsilon_2(D,D_{\pm z}),\delta)$-pDP,
%   	\end{enumerate}
%       	\vspace{-0.5em}
%   with    
%       	\vspace{-2.2em}
%   \begin{align*}
%   &\epsilon_2(o, D, D_{\pm z}) = \epsilon_2(D,D_{\pm z}) \\
%   =& \frac{\|\nabla \ell_z(\hat{\theta}^P)\|^2}{2\sigma_2^2}  + \frac{\|\nabla \ell_z(\hat{\theta}^P)\|\sqrt{2\log(2/\delta)}}{\sigma_2}.
%   \end{align*}
% \end{theorem}
% \begin{theorem}   	\label{thm:alg3_pdp}
% 	   	Let $\hat{\theta}^P$ be fixed, Algorithm~\ref{alg:Alg3} satisfies
% 	\vspace{-1em}
% 	\begin{enumerate}
% 		\itemsep0em
% 		\item $\epsilon_3(o,D,D_{\pm z})$-ex post pDP with probability $1-\delta$,
% 		\item $(\epsilon_3(D,D_{\pm z}),\delta)$-pDP,
% 	\end{enumerate}
%       	\vspace{-0.5em}
% with    
% %   Algorithm~\ref{alg:Alg3} satisfies $\epsilon_3(\cdot)$-ex post pDP with probability $1-\delta$; and also $(\epsilon_3(\cdot),\delta)$-pDP with
%  $
%  \epsilon_3(o, D,D_{\pm z}) =  \epsilon_3(D,D_{\pm z})  = \frac{\Delta_z^2}{2\sigma_3^2}  + \frac{\Delta_z\sqrt{2\log(2/\delta)}}{\sigma_3},$
%  where $\Delta_z  =  \dfrac{f''(x^T \theta) \mu_2(x)}{1 + f''(x^T \theta) \mu_1(x)}$, $\mu_1 = x^TH^{-1}x$ and $\mu_2=x^TH^{-2}x$. 
%   \end{theorem}
% 	The proofs of Theorem~\ref{thm:alg2_pdp} and \ref{thm:alg3_pdp} (which are deferred to the appendix) apply the pDP analysis of the Gaussian mechanism and an exact calculation of the perturbation vector resulting from adding or removing data point $z$. 
     
%   As we can see, the pDP losses of these two algorithms are comparable to that in $\epsilon_1(\hat{\theta}^P, D, z)$. Moreover, the quantities that are needed to compute these pDP losses of Algorithm~\ref{alg:Alg2}~and~\ref{alg:Alg3} are readily computable from the $z$ and the released values themselves, thereby avoiding the need for an \emph{infinite recursion} as we discussed in the third challenge.
   
   %Readers familiar with the DP literature may ask why we choose to release $H^{-1}$ rather than $H$, as the latter has a simpler summation form. We will see that releasing $H^{-1}$ directly allows us to obtain substantially smaller pDP losses.
    
%  \noindent\textbf{Calibrating noise to privacy budgets.} Algorithms~\ref{alg:Alg2} and \ref{alg:Alg3} take as input the noise parameters $\sigma_2$ and $\sigma_3$. Though we allow the noise parameters to be user-defined inputs, the data curator should set $\sigma_2, \sigma_3$ as usual to achieve a prescribed $(\epsilon, \delta)$-DP guarantee. Note that the data curator mustn't be tempted to calibrate the noise based on the per-instance sensitivity of a particular individual -- then the scale of the noise itself might reveal information about the individual that the algorithm intends to protect! 
 
%   \noindent\textbf{Confidence bounds.} In Algorithm~\ref{alg:Alg2} and \ref{alg:Alg3}, we focus on providing the plug-in estimators of the unknown quantities by the privately released values. Since we know the distribution of the noise exactly, we can also construct precise confidence intervals of around our released functions $\mu_1^P, \mu_2^P, \epsilon_3^P, q_2^P, q_3^P$ whenever a fixed $z$ is plug in to them. In the following we denote the upper and lower bounds of these quantities with an $\overline{\cdot}$ and $\underline{\cdot}$ respectively. These confidence bounds are used in Algorithm~\ref{alg:Alg4} and in the experiments, we provide detailed calculations of them in the supplementary materials.
    
%    We next present our algorithms to release the data-dependent quantities in $\epsilon_1(\hat{\theta}^P, D, z)$. As a note before we begin, Algorithms~\ref{alg:Alg2} and \ref{alg:Alg3} take as input the noise parameters $\sigma_2$ and $\sigma_3$. Though we allow the noise parameters to be user-defined inputs, the data curator should set $\sigma_2, \sigma_3$ as usual to achieve a prescribed $(\epsilon, \delta)$-DP guarantee. Note that the data curator mustn't be tempted to calibrate the noise based on the per-instance sensitivity of a particular individual -- then the scale of the noise itself might reveal information about the individual that the algorithm intends to protect!
    
%    The allotment of the privacy budget to Algorithms~\ref{alg:Alg1}, \ref{alg:Alg2} and \ref{alg:Alg3} is not an obvious choice. In Section~\ref{experiments} we offer some guidance on this matter based on our experimental results.

%    \begin{algorithm}[H]
%        \caption{Release $g^T \nabla \ell_z(\theta)$ from Algorithm~\ref{alg:Alg1}}
%        \label{alg:Alg2}
%        \begin{algorithmic}
%            \STATE {\bfseries Input:} Dataset $D$, privatized output $\hat{\theta}^P$, noise parameter $\sigma_2$, linear loss function $L(\theta; D) = \sum_i \ell_i(\theta)$, regularization parameter $\lambda$, convex and twice-differentiable regularizer $r$.
%            \STATE {\bfseries Output:} $q_2^P, \epsilon_2$.
%            \STATE Construct noise vector $e \sim \mathcal{N}(0, \sigma_2^2 I)$.
%            \STATE Set $g^P := \nabla L(\hat{\theta}^P; D) + \nabla r(\theta) + \lambda \hat{\theta}^P + e$.
%            \STATE Compute $q_2^P := (g^P)^T \nabla \ell_z(\hat{\theta}^P)$.
%            \STATE Set $\epsilon_2 := \frac{1}{\sigma^2}||\nabla \ell_z(\hat{\theta}^P)||_2 \sqrt{2 \log(1.25/\delta)}$.
%        \end{algorithmic}
%    \end{algorithm}

%\yw{You will notice that I modified Algorithm~\ref{alg:Alg2} and Algorithm~\ref{alg:Alg3} so that they return two things: (1) functions of $z$ that are necessary to compute an upper bound of the ex post pDP of Algorithm~\ref{alg:Alg1}; (2) high probability ex post pDP losses of itself according to Corollary~\ref{cor:highprob_pdp}.  I am using the $\overline{\mu}$ to denote an (high prob) upper bound  and $\underline{\mu}$ to denote a (high prob) lower bound of the quantity $\mu$.   Those ``error bars'' rely on e.g., Bernstein inequalities and should depend only on $z$ too, we need to work those out.}

%     \begin{algorithm}[t]
% 	\caption{Release $g$ for $g^T \nabla \ell_z(\theta)$ from Algorithm~\ref{alg:Alg1}}
% 	\label{alg:Alg2}
% 	\begin{algorithmic}
% 		\STATE {\bfseries Input:} Dataset $D$, privatized output $\hat{\theta}^P$, noise parameter $\sigma_2$, linear loss function $L(\theta; D) = \sum_i \ell_i(\theta)$, regularization parameter $\lambda$, convex and twice-differentiable regularizer $r$.
% 		\STATE {\bfseries Output:} $q_2^P(\cdot), \epsilon_2(\cdot)$.
% 		\STATE Construct noise vector $e \sim \mathcal{N}(0, \sigma_2^2 I)$.
% 		\STATE Set $g^P := \nabla L(\hat{\theta}^P; D) + \nabla r(\theta) + \lambda \hat{\theta}^P + e$.
% 		\STATE Set $q_2^P(\cdot)$ s.t. $q_2^P(z) = (g^P)^T \nabla \ell_z(\hat{\theta}^P)$.
% 		\STATE Set $\epsilon_2(\cdot)$ s.t. $\epsilon_2(z)= \frac{\|\nabla \ell_z(\hat{\theta}^P)\|^2}{2\sigma_2^2}  + \frac{\|\nabla \ell_z(\hat{\theta}^P)\|\sqrt{2\log(2/\delta)}}{\sigma_2}$.% according to \eqref{eq:pdp_gm} with $\Delta_z = \nabla \ell_z(\hat{\theta}^P)$.
% %		\STATE Set $\epsilon_2 := \frac{1}{\sigma^2}||\nabla \ell_z(\hat{\theta}^P)||_2 \sqrt{2 \log(1.25/\delta)}$.
% 	\end{algorithmic}
% \end{algorithm}


            %     \begin{algorithm}[t]
            % 	\caption{Release $H^{-1}$ for $\mu_1(x)$ from Algorithm~\ref{alg:Alg1}}
            % 	\label{alg:Alg3}
            % 	{\small
            % 		\begin{algorithmic}
            % 			\STATE {\bfseries Input:} Dataset $D$, %individual $z$'s data $z = (x, y)$, 
            % 			privatized output $\hat{\theta}^P$, noise parameter $\sigma_3$, linear loss function $L(\theta; D) = \sum_i \ell_i(\theta)$, regularization parameter $\lambda$, convex and twice-differentiable regularizer $r$.
            % 			\STATE {\bfseries Output:} %$\mu_1^P(\cdot), \mu_2^P(\cdot),
            % 			$q_3^P(\cdot)$%,\epsilon_3^P(\cdot)$.
            % 			\STATE Construct noise matrix $E$, where each entry is sampled i.i.d as $e_{ij} \sim \mathcal{N}(0, \sigma_3^2)$.
            % 			\STATE Set $(H^{-1})^P := (\nabla^2 L(\hat{\theta}^P; D) + \nabla^2 r(\hat{\theta}^P) +  \lambda I)^{-1} + E.$
            % 			\STATE Set  $q_3^P(\cdot)$ such that $q_3^P(z) =(H^{-1})^Px$.
            
            
            
%            			\STATE Set $\overline{\mu_1^P}(\cdot)$ s.t. $\overline{\mu_1^P}(z) = \min\{ \frac{\|x\|^2}{\lambda},  x^T(H^{-1})^P x\}$.
            			%
%            			\STATE Set $\epsilon_3^P(\cdot)$ s.t. $\epsilon_3^P(z) = \frac{\Delta_z^2}{2\sigma_3^2}  + \frac{\Delta_z\sqrt{2\log(2/\delta)}}{\sigma_3},$
%            			where $\Delta_z  =  \dfrac{f''(x^T \theta) \mu_2^P}{1 + f''(x^T \theta) \mu_1^P}$ with $\mu^P_1, \mu^P_2$ computed using 
%            			{\scriptsize
%            				\begin{equation*}
%            				\left\{
%            				\begin{aligned}
%            				\mu^P_1 :=& \max(0, x^T (H^{-1})^Px),\\
%            				\mu^P_2 :=& \min\left(\frac{\|x\|^2}{\lambda^2}, x^T[(H^{-1})^P]^T (H^{-1})^Px - \mathbb{E}\big[ x^TE^TEx\big]\right).
%            				\end{aligned}
%            				\right. 
%            				\end{equation*}
%            			}
%            			%	\dfrac{1}{\sigma^2}\dfrac{f''(x^T \theta) \mu_2^P}{1 + f''(x^T \theta) \mu_1^P}\sqrt{\log(1.25/\delta)}$ 



            % 		\end{algorithmic}
            % 	}
            % \end{algorithm}

    % \noindent\textbf{Joint differential privacy.} If we consider an extension of Algorithm~\ref{alg:Alg4} that publish the privacy reports to all $z\in \cD$, then by Theorem~\ref{thm:Alg1}, \ref{thm:alg2_pdp} and \ref{thm:alg3_pdp} implies an ex post and per-instance version of the joint DP \citep{kearns2014mechanism} via a generalized billboard lemma.  In order to avoid a lengthy detour, we provide more details about this connection in the appendix. Complementary to our methods satisfying joint pDP, we will consider a strict generalization of joint DP by analyzing the the privacy loss with respect to every fix set of colluding adversaries the same appendix.
    %Algorithm~\ref{alg:Alg2} is an application of the classical Gaussian mechanism, which calibrates the noise level according to the sensitivity of the output function. Conversely, \cite{wang2019per} shows that the per-instance privacy loss is proportional to the per-instance sensitivity. This observation forms the crux of our per-instance privacy analysis of Algorithms~\ref{alg:Alg2} and \ref{alg:Alg3}, along with the additional relaxation to joint differential privacy. 
    
    %Using joint per-instance DP, we can view $\epsilon_2^P(D, z)$ as an output of Algorithm~\ref{alg:Alg2} that is given privately to individual $z$. Clearly there will be no additional per-instance privacy loss to $z$ in the best-case scenario where no recipient $i$ of $\epsilon_2^P(D, z_i)$ reveals their private output. The joint per-instance differential privacy definition protects against the worst-case event that all others collude against $z$ by revealing their output.
%    
%    \subsubsection{Privacy guarantees of Algorithm~\ref{alg:Alg2}}
%    
%    \begin{theorem} 
%        \label{thm:alg2}
%        Algorithm 2 satisfies $(\epsilon_2(\cdot), \delta_2)$-joint per-instance differential privacy with
%        \begin{align*}
%            \epsilon_2(D, z) &=
%            \frac{||\nabla \ell_z(\hat{\theta}^P)||_2}{\sigma^2}\sqrt{2\log(1.25/\delta)}.
%        \end{align*}
%    \end{theorem}
%    
%    \begin{algorithm}[H]
%        \caption{Release $\mu_1(x)$ from Algorithm~\ref{alg:Alg1}}
%        \label{alg:Alg3}
%        \begin{algorithmic}
%            \STATE {\bfseries Input:} Dataset $D$, individual $z$'s data $z = (x, y)$, privatized output $\hat{\theta}^P$, noise parameter $\sigma_2$, linear loss function $L(\theta; D) = \sum_i \ell_i(\theta)$, regularization parameter $\lambda$, convex and twice-differentiable regularizer $r$.
%            \STATE {\bfseries Output:} $q_3^P, \epsilon_3^P$.
%            \STATE Construct noise matrix $E$, where each entry is sampled i.i.d as $e_{ij} \sim \mathcal{N}(0, \sigma_3^2)$.
%            \STATE Set $(H^{-1})^P := (\nabla^2 L(\hat{\theta}^P; D) + \nabla^2 r(\hat{\theta}^P) +  \lambda I)^{-1} + E.$
%            \STATE Compute $q_3^P :=(H^{-1})^Px$.
%            \STATE Set $\mu^P_1 := \max(0, x^T h^P)$.
%            \STATE Set $\mu^P_2 := (h^P)^Th^P - \mathbb{E}\big[ x^TE^TEx\big]$.
%            \STATE Set $\epsilon_3^P := \dfrac{1}{\sigma^2}\dfrac{f''(x^T \theta) \mu_2^P}{1 + f''(x^T \theta) \mu_1^P}\sqrt{\log(1.25/\delta)}$.
%        \end{algorithmic}
%    \end{algorithm}


%
%    
%    \subsubsection{Utility guarantees of Algorithm~\ref{alg:Alg2}}
%
%    \subsubsection{Privacy guarantees of Algorithm~\ref{alg:Alg3}}
%
%    \begin{theorem} 
%        \label{thm:alg3}
%        Algorithm 3 satisfies $(\epsilon_3(\cdot), \delta_3)$-joint per-instance differential privacy with
%        \begin{align*}
%            \epsilon_3(D, z) &=
%            \frac{1}{\sigma^2}\dfrac{f''(x^T \theta)\mu_2(x)}{1 + f''(x^T \theta) \mu(x)}\sqrt{2\log(1.25/\delta)}.
%        \end{align*}
%        where $\mu(x) = f''(x^T \theta)x^T(\nabla^2 L(\theta; D) + r(\theta) + \lambda I)^{-1} x$ and $\mu_2(x) = f''(x^T \theta)x^T(\nabla^2 L(\theta; D) + r(\theta) + \lambda I)^{-2} x$ are the out-of-sample leverage and quadratic leverage scores.
%    \end{theorem}
%    
%    \subsubsection{Utility guarantees of Algorithm~\ref{alg:Alg3}}


% \begin{proposition}[Uniform multiplicative approximation]\label{prop:utility_H_large_lambda}
% 	Denote $H := \nabla^2 J(\hat{\theta}^P; D)$. If $\lambda_{\min}(H) \geq  2 \sigma_2 F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$, then with probability $1-\rho$, for all $x\in \R^d$ simultaneously 
% 	$$
% 	\frac{1}{2}  x^T(\hat{H}^P)^{-1}x \leq x^TH^{-1}x \leq \frac{3}{2}x^T(\hat{H}^P)^{-1}x.
% 	$$
% \end{proposition}

==> Privately Publishable Per-instance Privacy/subsections/utility.tex <==
% !TEX root = ../main.tex

The privatized output should be a good approximation to the original input, in addition to providing strong privacy guarantees. Here we'll present high-probability utility bounds for Algorithms~\ref{alg:Alg2} and \ref{alg:Alg3}.

\begin{theorem}[Utility bound for Algorithm~\ref{alg:Alg2}]
    \label{thm:utility_alg2}
    With probability $1 - \delta$, the output $(g^P)^T \nabla \ell_z(\hat{\theta}^P)$ of Algorithm~\ref{alg:Alg2} satisfies
    \begin{align*}
        \big|(g^P)^T\ell_z(\hat{\theta}^P) - g^T\ell_z(\hat{\theta}^P)\big| &\leq \sigma_2 || \nabla \ell_z(\hat{\theta}^P) ||_2 \sqrt{2 \log(2/\delta)}.
    \end{align*}
\end{theorem}
%
%\begin{theorem}[Utility bound for Algorithm~\ref{alg:Alg3}]
%\label{thm:utility_alg3}
% With probability $1 - \delta_3$, the quantity $\Delta_z$ of Algorithm~\ref{alg:Alg3} satisfies
%    \begin{align*}
%        &\left|\dfrac{f''(x^T \hat{\theta}^P)\mu_2^P}{1 + f''(x^T \hat{\theta}^P)\mu_1^P} - \dfrac{f''(x^T \hat{\theta}^P)\mu_2}{1+ f''(x^T \hat{\theta}^P)\mu_1} \right|  \leq \\
%        &\:\:\sigma_3 || x || \sqrt{2 \mu_2(x) \log(2/\delta)}  \\&\:\:+2 \sigma_3 ||x|| \sqrt{d} \log(1/\delta) + 2 \sigma_3 ||x|| \ln(1/\delta).
%    \end{align*}
%\end{theorem}

\begin{theorem}[Key error bounds for Algorithm~\ref{alg:Alg3}]
	\label{thm:utility_alg3}
	With probability $1 - \delta$, the quantity $\Delta_z$ of Algorithm~\ref{alg:Alg3} satisfies
	\begin{align*}
	\dfrac{f''(x^T \hat{\theta}^P)\underline{\mu_2^P}}{1 + f''(x^T \hat{\theta}^P)\overline{\mu_1^P}} \leq \Delta_z    \leq  \dfrac{f''(x^T \hat{\theta}^P)\overline{\mu_2^P}}{1 + f''(x^T \hat{\theta}^P)\underline{\mu_1^P}},
	\end{align*}
	where $\underline{\mu_2^P}, \overline{\mu_2^P},\underline{\mu_1^P},\overline{\mu_1^P}$ are valid $1-\delta/4$ upper and lower bounds of $\mu_2$ and $\mu_1$ at $z$.
\end{theorem}
We will denote the above  bounds $\overline{\Delta}_z$ and $\underline{\Delta}_z$.


==> sections/experiments_original.tex <==
% !TEX root = ../main.tex

We evaluate our methods to release the pDP losses across a variety of datasets, using linear and logistic regression as case studies.

\textbf{Experimental Setup}\: Throughout, we set $\delta = 10^{-6}$ (failure probability of Algorithm ~\ref{alg:Alg1}, i.e. objective perturbation) and $\rho = 10^{-6}$ (failure probability of Algorithm \ref{alg:privacy_report} that releases a private upper bound on the pDP loss). Our choice of $\sigma$ depends on $\epsilon_1$ and follows the requirements for objective perturbation stated in Theorem \ref{thm:alg1} to achieve DP.  Unless otherwise specified, we set $\lambda$ as described in Algorithm \ref{alg:privacy_report}. We don't use any additional regularization, i.e. $r(\theta) = 0$. The noise parameters $\sigma_2, \sigma_3$ are each calibrated according to the analytic Gaussian mechanism of \citep{balle2018improving}, with an equal privacy budget allotted to each private release. In other words, Algorithm \ref{alg:Alg1} which releases $\hat{\theta}^P$ has a budget of $\epsilon_1$; Algorithm \ref{alg:privacy_report} which releases $\overline{\mu^P}(\cdot)$ and $\overline{g^P}(\cdot)$ has a budget of $2\epsilon_1$; and therefore the combined privacy budget of objective perturbation and releasing the associated pDP losses is equal to $3 \epsilon_1$.

\textbf{Datasets}
%kidney, synthetic, credit, liver, wine
For experiments related to linear regression, we use the wine quality dataset \citep{Dua:2019} from the UCI Machine Learning Repository. We also evaluate our methods on synthetic data generated by sampling $x_i, \theta \sim \mathcal{N}(0, I_d)$ and normalizing each $x_i \in X$ so that $||x_i||_2 = 1$. The unperturbed response variable $Y \in \mathbb{R}^n$ is then determined as $Y = X \theta$ and rescaled so that each $y_i \in [0, 1]$.

We use three UCI datasets to test our methods on logistic regression: the credit card default dataset \citep{yeh2009comparisons}, the chronic kidney disease dataset and the liver disorders dataset \citep{Dua:2019}. In addition, we generate synthetic data by sampling  $x_i, \theta \sim \mathcal{N}(0, I_d)$ and determining each $y_i$ as
%\centerline{
$$y_i = \begin{cases} 
        1 & \text{ if } \texttt{sigmoid}(x_i^T\theta) > 0.5, \\ 
        0 & \text{ otherwise.} \end{cases}$$
        %}

\subsection{Stronger regularization does not worsen model utility}
% logistic regression
% explain lambda_inflate
% star denotes the actual inflation value (how many times larger \lambda_{adapt} is than \lambda_{obj})
% can see it has minimial effect on the 0-1 loss of the model
\begin{minipage}{.4\textwidth}
Algorithm ~\ref{alg:privacy_report} requires a larger $\lambda$ than suggested by Theorem $\ref{thm:alg1}$ in order to achieve a uniform multiplicative approximation of $\mu(\cdot)$.  
We investigate the effect of stronger regularization on the utility of a private logistic regression model applied to a synthetic dataset ($n = 1000, d = 50$), for several settings of $\epsilon_1$. Since each value of $\epsilon_1$ demands a different minimum value of $\lambda$ in order to achieve $(\epsilon_1, \delta)$-differential privacy, we compare via "$\lambda$-inflation": a measure of how many times larger we set $\lambda$ than its minimum value required to achieve the worst-case DP bound of objective perturbation.
\end{minipage}
\hspace{.2cm}\begin{minipage}{.6\textwidth}
\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/lambda_utility.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Utility of Obj-Pert with larger $\lambda$.}
  \label{fig:lambda_utility}
\end{figure}
\end{minipage}

  E.g., for logistic regression the objective perturbation mechanism requires $\lambda \geq \frac{1}{2\epsilon}$, and so in Figure ~\ref{fig:lambda_utility} a $\lambda$-inflation value of 10 means that we set $\lambda = \frac{5}{\epsilon}$. For each $\lambda$-inflate value $c$ , we run Algorithm \ref{alg:Alg1} with $\lambda = c \lambda_{\texttt{Obj-Pert}}$.  In particular, the star symbol marks the level of $\lambda$-inflation enforced by Algorithm ~\ref{alg:privacy_report}. The experimental results summarized in Figure ~\ref{fig:lambda_utility} show that the performance of the private logistic regression model (as measured by the 0-1 loss) remains roughly constant across varying scales of $\lambda$.


\subsection{Comparison of data-independent and data-dependent bounds}

Algorithm ~\ref{alg:privacy_report} presents two approaches to releasing a private upper bound of $\epsilon_1(\cdot)$, the pDP loss of releasing $\hat{\theta}^P$ from Algorithm ~\ref{alg:Alg1}. The data-independent approach bounds the pDP loss using only individual $z$'s own data as well as publicly-known parameters of the algorithm ($\rho, \sigma, \lambda$). The data-dependent approach privatizes the quantities $\mu(\cdot)$ and $g(\cdot) := \nabla J(\hat{\theta}^P; D)^T \nabla \ell(\hat{\theta}^P; z)$ that depend on the entire dataset. While the data-dependent approach can more accurately release $\overline{\epsilon_1^P}(\cdot)$, it suffers an additional privacy loss which could negate the savings of a more accurate bound on the pDP loss of Algorithm ~\ref{alg:Alg1}. It is therefore of interest to us to investigate the trade-offs of both approaches.

First, we run both the data-independent and -dependent variations of Algorithm ~\ref{alg:Alg1} with privacy parameters set to achieve $\epsilon_1 = \epsilon_2 = \epsilon_3 = 1$, as described in the experimental setup. Figure ~\ref{fig:ep1_compare} compares the distributions of the true pDP loss $\epsilon_1(\cdot)$ and its privately released upper bound $\overline{\epsilon_1^P}(\cdot)$ using both the data-independent and -dependent approaches. We see that for the same privacy budget $\epsilon_1 = 1$ allotted to Algorithm ~\ref{alg:Alg1} (indicated by the red line), the data-dependent upper bound is significantly tighter than the data-independent upper bound. However, Figure ~\ref{fig:ep1_compare} doesn't take into account the additional privacy loss incurred by using the data-dependent version of Algorithm ~\ref{alg:privacy_report}.

\begin{figure}[H]
  \centering
\includegraphics[width=\textwidth]{experiments/ep1_datasets.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Comparison of pDP losses and data-independent and -dependent upper bounds}
  \label{fig:ep1_compare}
\end{figure}

Figure ~\ref{fig:ep1_ep23_compare} includes the additional per-instance privacy loss of Algorithm ~\ref{alg:privacy_report} (for the data-independent version, we simply have $\epsilon_2(\cdot) = \epsilon_3(\cdot) = 0$). When considering the combined pDP loss of running Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report}, the data-independent bound is tighter. However, it is perhaps unfair of us to compose the \emph{ex-post} pDP loss of Algorithm ~\ref{alg:Alg1} with the \emph{ex-ante} pDP loss of Algorithm ~\ref{alg:privacy_report}, particularly given that the the \emph{ex-ante} pDP loss of Algorithm ~\ref{alg:privacy_report} has a necessary dependence on the order of $\sqrt{2\log(1/\delta)}$. In the appendix, we explore how to allocate the privacy budget between Algorithms ~\ref{alg:Alg1} and ~\ref{alg:privacy_report} in order to achieve a more favorable trade-off between the data-independent and data-dependent approaches.

Based on our theory and experiments, our recommendation is to use data-independent bounds if $\lambda$ is large (the second or the third term dominates $\epsilon_1(\cdot)$). 
The data-dependent bound (and the adaptive algorithm presented in the appendix) may be preferred if $\lambda$ is small and the $-\log(1-\mu(\cdot))$ term dominates  the $\epsilon_1(\cdot)$). 
Since the additional overhead of the data-dependent approach increases only the second and third term of $\epsilon_1(\cdot)$, only when the first term dominates, will the improvement from the data-dependent bound be significant enough to outweigh the incurred additional pDP losses.

\begin{figure}[H]
  \centering
    \includegraphics[width=\textwidth]{experiments/ep1_datasets_ep23.pdf}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Comparison of the pDP losses with the additional overhead added.}
  \label{fig:ep1_ep23_compare}
\end{figure}


% \subsection{True pDP loss $\epsilon_1$ vs. released bound $\tilde{\epsilon_1}$}

% \label{exp:first}
% In this experiment we use a synthetic dataset, sampling $\theta \sim \mathcal{N}(0, 1)$, sampling $X \in \mathbb{R}^{n \times d}$ from the $d$-dimensional unit ball. $Y$ is then a deterministic function of $X$ and $\theta$ such that Pr[$Y = 1$] = \texttt{sigmoid}($X^T \theta) + E$ for noise matrix $E$. Figure ~\ref{fig:histograms} plots the pDP distributions for the true $\epsilon_1$ and its data-independent bound $\tilde{\epsilon}$ calculated according to Algorithm ~\ref{alg:privacy_report}, demonstrating both that the true \emph{ex-post} pDP loss is an order of magnitude improvement compared to the worst case DP bound $\epsilon$, and that the data-independent bound provides a good approximation to the true pDP loss.

% Generate random \theta of dimensionality d, X of dimensionality n by d, Y = X^T \theta + noise.


% dimension logistic
% generate data with "generate_data" function (describe)
% vary d = [1, ..50, 60] and calculate 1) max_i \epsilon_1(i) and \epsilon_1^P(i) using data-independent bound...same for best-case and median case

% true_release_comp
% kidney dataset?
% for varying levels of \epsilon, do objective perturbation as described in Theorem ? and calculate pDP distributions for the true and released values of \epsilon_1, using data-independent bounds

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/true_release_comp.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{pDP distributions for the true $\epsilon_1$ and its data-independent bound.}
%   \label{fig:histograms}
% \end{figure}

% \subsection{Dimension}

% We generate synthetic data as described in the previous experiment, this time varying $d \in [1, 5, 10, 20, 30, 40, 50, 60]$. We choose $\epsilon = 0.5$ as the DP bound and $\delta = 10^{-3}$, and set $\sigma, \lambda$ according to Theorem ~\ref{thm:alg1}. Figure ~\ref{fig:dimension} plots the true worst-, best- and median-case \emph{ex-post} pDP loss over all individuals $z$ against its data-independent counterpart (i.e., the worst-case pDP loss is calculated as $\max_{z \in D} \epsilon(\cdot, D_{\pm z})$ and the worst-case data-independent bound as $\max_{z \in D} \Tilde{\epsilon}(\cdot, z)$).

% \begin{figure}[H]
%   \centering
%     \includegraphics[width=\textwidth]{experiments/dimension_logistic.pdf}
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{pDP losses across varying data dimensions.}
%   \label{fig:dimension}
% \end{figure}



==> subsections/overflow_algorithms_and_proofs.tex <==
% !TEX root = ../main.tex

        \begin{algorithm}[H]
        \caption{Dataset-dependent privacy report for \texttt{Obj-Pert} on GLMs}
        \label{alg:dataset_dependent_report}
        \begin{algorithmic}
            \STATE {\bfseries Input:} $\hat{\theta}^p$ from \texttt{Obj-Pert}, noise parameter $\sigma_1,\sigma_2,\sigma_3$; regularization parameter $\lambda$; Hessian $H := \sum_i\nabla^2\ell_i(\hat{\theta}^p) + \lambda I_d$.
            \STATE {\bfseries Output:} Reporting function $\tilde{\epsilon}: (x,y),\delta \rightarrow \R_+^2$
            \STATE Privately release $\hat{H}^p$ by Algorithm~\ref{alg:release_H} with parameter $\sigma_2$. 
             \STATE Sets $\epsilon_2(\cdot))$  according to Theorem~\ref{thm:pdp_of_H_lambda_min}.
            \STATE Set $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$.
            $\tau$ is on the order of $O(\sqrt{d}(1 + \log(C/\rho)^{3/2}))$ by Lemma~\ref{lem:lambda_GOE}.
            \STATE \IF{$\lambda \geq  2 \tau \sigma_2$}
            \STATE Set $\overline{\mu^p}(x) = \min\{\frac{3}{2}x^T [\hat{H}^p]^{-1} x,\frac{\|x\|^2}{\lambda}\}$
            \STATE Set $\epsilon_3(\cdot)\equiv 0$ 
            \ELSE
            \STATE Privately release $\hat{\lambda}_{\min}^p = \lambda_{\min} + \cN(0,\sigma_3^2)$.
              \STATE Sets $\epsilon_3(\cdot))$  according to Theorem~\ref{thm:pdp_of_H_lambda_min}.
            \STATE \IF{$\underline{\hat{\lambda}_{\min}^p}:=\hat{\lambda}_{\min}^p - \sigma_3 F_{\cN(0,1)}^{-1}(1-\rho/2)\geq  2 \tau\sigma_2$}
            \STATE Set $\overline{\mu^p}(x) = \min\{\frac{3}{2} x^T [\hat{H}^p]^{-1} x,\frac{\|x\|^2}{\max\{\lambda, \underline{\hat{\lambda}_{\min}^p}\}}\}$
            \ELSE 
            \STATE Set $\overline{\mu^p}(x) = \min\{\frac{\lambda + \tau \sigma_2}{\lambda } x^T (\hat{H}^p +  \tau \sigma_2 I_d)^{-1} x,\frac{\|x\|^2}{\max\{\lambda, \underline{\hat{\lambda}_{\min}^p}\}}\}.$
            \ENDIF 
            \ENDIF
            \STATE Set $\overline{\epsilon_1^p}(z):= \max\left\{
            \left|-\log \big(1 \pm f''(z,\hat{\theta}^p)\overline{\mu^p}(x) \big) + \frac{|f'(z,\hat{\theta}^p)|^2||x||^2}{2\sigma_1^2}  \pm  \frac{|f'(z,\hat{\theta}^p)|||x|| F_{\cN(0,1)}^{-1}(1-\nicefrac{\rho}{2})}{\sigma_1} \right|\right\}$.
            \yw{The maximum above is for the two possiblities, $\pm$.}
            \STATE Set $\tilde{\epsilon}_1(\cdot) = (\overline{\epsilon_1^p}(\cdot), \epsilon_2(\cdot) + \epsilon_3(\cdot))$
            \yw{Let's drop the lower bound and focus on separately reporting the released ex post-PDP parameter and then report the addtional overhead separately.}
            \yw{We could also simplify this algorithm so we only talk about the setting with sufficiently large $\lambda$.  Then we can say that we also propose a more adaptive algorithm that allows us to release valid bounds for all choices of $\lambda >0$ and adapt to well-conditioned $H$. Say that it is more tedious thus we include it only in the appendix.  Notice that the theorems that I stated are all about the case when $\lambda$ is large.}
            \vspace*{1mm}
        \end{algorithmic}
    \end{algorithm}
    
       Note that the pDP functions of the reporting algorithm $\epsilon_2(\cdot), \epsilon_3(\cdot)$ does not depend on the dataset, and thus is not required to be separately released.
    
       \begin{proposition}[Uniform privacy report]
    With probability $1-2\rho$,  \emph{simultaneously} for all $n$ users in the dataset, $\epsilon_1(z,\hat{\theta}^p) \leq \overline{\epsilon_1}^P(z,\hat{\theta}^p) \leq 12 \sqrt{\log n} \epsilon_1(z,\hat{\theta}^p)$
    
    If we, instead, use $\frac{|f'(z,\hat{\theta}^p)|\|x\|_1\sqrt{2\log(2d/\rho)}}{\sigma_1} $ to replace the third-term in $\overline{\epsilon^p}_1$, then with probability $1-2\rho$, \emph{simultaneously} for all $x\in\cX$, the ex post pDP report $\overline{\epsilon^p}_1$ satisfies that
    $$\epsilon_1(z,\hat{\theta}^p) \leq \overline{\epsilon^p}_1(z,\hat{\theta}^p) \leq 12 \sqrt{d\log d}\epsilon_1(z,\hat{\theta}^p).$$ 
        % \item With probability $1-\rho$, \emph{uniformly} For all $(x,y)\in\R^d\times \mathcal{Y},$ the \emph{ex post} pDP loss 
        % $\epsilon(z,\hat{\theta}^p) \leq $
    \end{proposition}
    \begin{proof}
    We note that the approximation of $\mu_x$ is uniform for all $x$. It remains to consider a uniform bound for the third term over the randomness of ObjPert. The first statement follows by taking union bound. And the second result is achieved by Holder's inequality,  the concentration of max of iid Gaussian, and that $\|x\|_1\leq \sqrt{d}\|x\|_2$. 
    \end{proof}
    
     \begin{proposition}[Uniform multiplicative approximation of a regularized estimator]\label{prop:utility_H_regularized}
 Let $\hat{H}^P$ be constructed through Algorithm~\ref{alg:release_H} with parameter $\sigma_2$ and let $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$. Then with  probability $1-\rho$, for all $x\in \R^d$
     $$ x^T(\hat{H}^P + \tau \sigma_2 I_d)^{-1}x \leq \mu(x) \leq \frac{\lambda + 2\tau\sigma_2}{\lambda} x^T(\hat{H}^P + \tau\sigma_2 I_d)^{-1}x. $$
 \end{proposition}
 \begin{proof}
 We choose $\tau = F_{\lambda_1(\mathrm{GOE}(d))}^{-1}(1-\rho/2)$. With probability $1-\rho/2$, the largest eigenvalue is smaller than $\tau$.
 Similarly, by symmetry, with probability $1-\rho/2$, the smallest eigenvalue is larger than $-\tau$.
 By a union bound,  we have that with probability $1-\rho$
  $\|Z\|_2\prec \tau,$ i.e., $-\tau I_d \prec Z\prec \tau I_d$.
\begin{align*}
H&\prec H + Z + \tau \sigma_2 I_d \prec H + 2\tau \sigma_2 I = \nabla^2 L(\hat{\theta}^P) + \lambda I_d + 2\tau\sigma_2 I_d \\
&\prec \frac{\lambda + 2\tau\sigma_2}{\lambda}(\nabla^2 L(\hat{\theta}^P) + \lambda I_d) = \frac{\lambda + 2\tau\sigma_2}{\lambda} H.
\end{align*} 
Take inverse on both sides, we get
$$
\frac{\lambda}{\lambda + 2\tau\sigma_2}H^{-1} \prec (\hat{H}^P + \tau \sigma_2 I_d)^{-1} \prec H^{-1}.
$$
Thus for all $x\in \R^d$,
$x^T(\hat{H}^P + \tau \sigma_2 I_d)^{-1}x \leq x^T H^{-1}x \leq \frac{\lambda + 2\tau \sigma_2}{\lambda} x^T(\hat{H}^P + \tau \sigma_2 I_d)^{-1}x.$
\end{proof}
 

The AnalyzeGauss algorithm however uses a slightly different Gaussian random matrix to privately release the upper-triangular part of $H$ with the standard Gaussian mechanism.
\begin{proposition}[Largest eigenvalue of the noise matrix of AnalyzeGauss]\label{lem:spectral_norm_analyzgauss}
Let $A$ be a symmetric Gaussian random matrix with iid entries drawn from $\cN(0,\sigma^2)$ on the upper triangular part of the matrix, then there exists a universal constant $C'$ such that with probability $1-\delta$
$$
\|A\|_2  \leq \sigma \sqrt{d}(3\sqrt{2} +C'(\log(\max\{2d,2C\}/\delta))^{2/3}.
$$
\end{proposition}
\begin{proof}
Let us construct 
$\tilde{A}= A + D $
where $D$ is the diagonal matrix where $D_{ii} = A_{ii} (\sqrt{2}-1)$.  Clearly, $\tilde{A}$ is a Gaussian orthogonal ensemble. Thus by Lemma~\ref{lem:max_of_subgaussian}, Lemma~\ref{lem:lambda_GOE} and the triangular inequality
$$
\|A\|_2 \leq \|\tilde{A}\|_2 + \|D\|_2 \leq \sqrt{2}\left(2 + \big(\frac{(\log(2C/\delta))}{c d}\big)^{2/3}\right) \sqrt{d\sigma^2} + \sigma (\sqrt{2}-1)\sqrt{2\log (2d/\delta)}.
$$
To get the desired result, we can take $\frac{\log(2C/\delta)}{cd} \leq \frac{\log(2C/\delta)}{c}$ (since $d\geq 1$) and that $\sqrt{x} \leq 1 + (x)^{2/3}$ for all $x>0$. $C'$ can be taken as $c^{-2/3}+(2-\sqrt{2})$. 
\end{proof}

\begin{remark}
Instead of ``analyze-gauss'' noise, it is arguably more natural to add a GOE noise where the diagonal elements receive a variance that is twice as large. This is because the sensitivity of the upper-triangular part of the matrix $H$ is naturally measured in terms of an $A$-norm where $A\in \R^{(\frac{d^2}{2}+d/2)\times (\frac{d^2}{2}+d/2)}$ is a diagonal matrix with all coordinates corresponding to the off-diagonal elements $H$ being $2$ and those cooresponding to the diagonal elements of $H$ being $1$. 
Let the perturbation (due to adding or removing one data point) being $xx^T$ and let $\Delta_x\in \R^{\frac{d^2}{2}+d/2}$ denotes the vectorized version of the upper triangular region of $xx^T$, then it is clear that $\|\Delta_x\|_A =  \|x\|^2$.
The corresponding multi-variate Gaussian mechanism add noises with covariance matrix $A^{-1}$, which involves adding twice as large a noise to the diagonal elements, i.e., the noise is a GOE random matrix! 
\end{remark}



\section{New method for privately releasing leverage scores}

% The new algorithm releases $H$ by a Gaussian mechanism.
% $$
% \hat{H}^p = H + Z
% $$
% where $Z$ is a symmetric Gaussian noise.


    \begin{algorithm}[H]
        \caption{ Release $H$ (a natural variant of ``Analyze-Gauss'') }
        \label{alg:release_H}
        \begin{algorithmic}
            \STATE{{\bfseries Input:} Dataset $D$, noise parameter $\sigma_2$, $H  = \sum_{i=1}^n \nabla^2\ell(z_i, \hat{\theta}^P) + \lambda I_d$.}
            \STATE{{\bfseries Output:} $\hat{H}^P$.}
           \STATE{Draw a  Gaussian random matrix $Z\in \R^{d\times d}$ with $Z_{i,j}\sim \cN(0,\sigma_2^2)$ independently.}
           \STATE{Output $\hat{H}^P = H + \frac{1}{\sqrt{2}}(Z + Z^T)$.}
        \end{algorithmic}
    \end{algorithm}
    
    \begin{algorithm}[H]
                        \caption{ Releasing the smallest eigenvalue of $H$ }                \label{alg:lambda_min}
        \begin{algorithmic}
            \STATE{{\bfseries Input:} Dataset $D$, noise parameter $\sigma_3$, $\lambda_{\min}$ denoting the smallest eigenvalue of $H$.}%  = \sum_{i=1}^n \nabla^2\ell(z_i, \hat{\theta}^P) + \lambda I_d$.}
            \STATE{{\bfseries Output:} $\hat{\lambda}_{\min}^P$.}
           \STATE{Output $\hat{\lambda}_{\min}^P = \lambda_{\min} + \cN(0,\sigma_3^2)$ .}
        \end{algorithmic}
    \end{algorithm}

\begin{theorem}\label{thm:pdp_of_H_lambda_min}
    Algorithm~\ref{alg:release_H} satisfies pDP with 
    $$
    \epsilon_2(z,\delta) = \frac{(f^{''}(x,\hat{\theta}^p))^2\|x\|^4}{4\sigma_2^2} +  \frac{f^{''}(x,\hat{\theta}^p)\|x\|^2\sqrt{\log(1/\delta)}}{\sigma_2},
    $$
    and $\hat{H}^p$ satisfies ex post pDP of the same $\epsilon$ with probability $1-2\delta$.
    
    Algorithm~\ref{alg:lambda_min} satisfies pDP with 
    $$
    \epsilon_3(z,\delta) = \frac{(f^{''}(x,\hat{\theta}^p))^2\|x\|^4}{2\sigma_3^2} +  \frac{f^{''}(x,\hat{\theta}^p)\|x\|^2\sqrt{2\log(1/\delta)}}{\sigma_3},
    $$
\end{theorem}
\begin{proof}
Algorithm~\ref{alg:release_H} is equivalent to releasing the vector 
$
[f_1, f_2]
$
using a standard Gaussian mechanism with $\cN(0,\sigma_2^2 I_{\frac{d^2}{2}+d/2})$, where $f_1\in\R^d$ is the diagonal of $H/\sqrt{2}$ and $f_2\in\R^{(d^2-d)/2}$ is the vectorized  the strict upper triangular part of $H$.

The per-instance L2-sensivitiy of $[f_1,f_2]$ is 
\begin{align*}
\|\Delta_x\|_2 &= f''(z,\hat{\theta}^p)\sqrt{\sum_{1\leq i<j\leq d}x_i^2x_j^2 + \sum_{k=1^d} x_{k,k}^4 (1/\sqrt{2})^2} \\
&= f''(z,\hat{\theta}^p)\sqrt{\frac{1}{2}\sum_{1\leq i,j\leq d}( x_i^2x_j^2 + \sum_{k=1^d} x_{k,k}^4} \\
&= \frac{f''(z,\hat{\theta}^p)}{\sqrt{2}}\|xx^T\|_F= \frac{f''(z,\hat{\theta}^p)}{\sqrt{2}}\|x\|_2^2.
\end{align*}
The result then follows from an application of the pDP computation of the Gaussian mechanism. \yw{Add the reference to the theorem of the Gaussian mechanism.}

To see the second statement, observe that it is a standard univariate Gaussian mechanism. By Weyl's lemma, the smallest singular value satisfies a perturbation bound of $f''(z,\hat{\theta}^p)\|xx^T\|_2 = f''(z,\hat{\theta}^p)\|x\|^2$, since the per-example Hessian is rank-1 in GLM. The stated result again follows from the theorem of the Gaussian mechanism.
\end{proof}

% to go with universal constant proof
  \begin{corollary}[The additional privacy cost]
    If we calibrate $\sigma_2$ such that the Algorithm~\ref{alg:dataset_dependent_report} satisfies the same $(\epsilon,\delta)$-DP as Algorithm~\ref{alg:Alg1}, i.e., when $\epsilon<1$, we could choose $\sigma_2 = \frac{\rho_{\max}}{\epsilon}\sqrt{2\log(1.25/\delta)}$ \footnote{We can alternatively use the optimal calibration via the analytical Gaussian mechanism~\citep{balle2018improving} (or equivalently via GDP) for a tighter calibration that applies to all $\epsilon\geq 0$.}. Then Algorithm~\ref{alg:dataset_dependent_report} satisfies $(\epsilon(z),\delta)$-pDP with
        $$
        \epsilon(z) =\frac{\epsilon^2 (f'')^2\|x\|^4}{8 \rho_{\max}^2 \log(1.25/\delta)} + \frac{\epsilon (f'')\|x\|^2}{\rho_{\max} \sqrt{2}}.$$
    For those cases when $ \frac{(f'')\|x\|^2}{\rho_{\max}}\leq  \frac{|f'|\|x\|}{\beta}$ (which is the case in logistic regression for all $x$ s.t., $\|x\|\leq 1$), the additional overhead in releasing a dataset-dependent pDP is smaller than the ex post pDP bound in Theorem~\ref{thm:pdp_alg1_general}.
    \end{corollary}
    


==> subsections/utility.tex <==
% !TEX root = ../main.tex

The privatized output should be a good approximation to the original input, in addition to providing strong privacy guarantees. Here we'll present high-probability utility bounds for Algorithms~\ref{alg:Alg2} and \ref{alg:Alg3}.

\begin{theorem}[Utility bound for Algorithm~\ref{alg:Alg2}]
    \label{thm:utility_alg2}
    With probability $1 - \delta$, the output $(g^P)^T \nabla \ell_z(\hat{\theta}^P)$ of Algorithm~\ref{alg:Alg2} satisfies
    \begin{align*}
        \big|(g^P)^T\ell_z(\hat{\theta}^P) - g^T\ell_z(\hat{\theta}^P)\big| &\leq \sigma_2 || \nabla \ell_z(\hat{\theta}^P) ||_2 \sqrt{2 \log(2/\delta)}.
    \end{align*}
\end{theorem}
%
%\begin{theorem}[Utility bound for Algorithm~\ref{alg:Alg3}]
%\label{thm:utility_alg3}
% With probability $1 - \delta_3$, the quantity $\Delta_z$ of Algorithm~\ref{alg:Alg3} satisfies
%    \begin{align*}
%        &\left|\dfrac{f''(x^T \hat{\theta}^P)\mu_2^P}{1 + f''(x^T \hat{\theta}^P)\mu_1^P} - \dfrac{f''(x^T \hat{\theta}^P)\mu_2}{1+ f''(x^T \hat{\theta}^P)\mu_1} \right|  \leq \\
%        &\:\:\sigma_3 || x || \sqrt{2 \mu_2(x) \log(2/\delta)}  \\&\:\:+2 \sigma_3 ||x|| \sqrt{d} \log(1/\delta) + 2 \sigma_3 ||x|| \ln(1/\delta).
%    \end{align*}
%\end{theorem}

\begin{theorem}[Key error bounds for Algorithm~\ref{alg:Alg3}]
	\label{thm:utility_alg3}
	With probability $1 - \delta$, the quantity $\Delta_z$ of Algorithm~\ref{alg:Alg3} satisfies
	\begin{align*}
	\dfrac{f''(x^T \hat{\theta}^P)\underline{\mu_2^P}}{1 + f''(x^T \hat{\theta}^P)\overline{\mu_1^P}} \leq \Delta_z    \leq  \dfrac{f''(x^T \hat{\theta}^P)\overline{\mu_2^P}}{1 + f''(x^T \hat{\theta}^P)\underline{\mu_1^P}},
	\end{align*}
	where $\underline{\mu_2^P}, \overline{\mu_2^P},\underline{\mu_1^P},\overline{\mu_1^P}$ are valid $1-\delta/4$ upper and lower bounds of $\mu_2$ and $\mu_1$ at $z$.
\end{theorem}
We will denote the above  bounds $\overline{\Delta}_z$ and $\underline{\Delta}_z$.

